SmartPortraits: Depth Powered Handheld Smartphone Dataset of Human Portraits for State Estimation, Reconstruction and Synthesis

We present a dataset of 1000 video sequences of human portraits recorded in real and uncontrolled conditions by using a handheld smartphone accompanied by an external high-quality depth camera. The collected dataset contains 200 people captured in different poses and locations and its main purpose is to bridge the gap between raw measurements obtained from a smartphone and downstream applications, such as state estimation, 3D reconstruction, view synthesis, etc. The sensors employed in data collection are the smartphone's camera and Inertial Measurement Unit (IMU), and an external Azure Kinect DK depth camera software synchronized with sub-millisecond precision to the smartphone system. During the recording, the smartphone flash is used to provide a periodic secondary source of lightning. Accurate mask of the foremost person is provided as well as its impact on the camera alignment accuracy. For evaluation purposes, we compare multiple state-of-the-art camera alignment methods by using a Motion Capture system. We provide a smartphone visual-inertial benchmark for portrait capturing, where we report results for multiple methods and motivate further use of the provided trajectories, available in the dataset, in view synthesis and 3D reconstruction tasks.

==> CVPR'21 Avatar dataset (Camera Ready)/src/01_intro.tex <==
% Notes
% infrared without dash
% the modern smartphone depth images are still not as high-quality as external depth sensors - comparison of images with sensor
\section{Introduction}
\label{sec:intro}

% What is the problem. Overlap between VIO sequences and people recording. This dataset meets both requirements with smartphone data
Realistic rendering of people, and in general of objects, has recently achieved an unprecedented level of detail and realism \cite{mildenhall2020nerf, lombardi2019neuralvolumes, shysheya2019textured, gafni2021dynamic, zakharov2020fast, wang2021learning, Zakharov2019talking, aliev2020neural} with potential groundbreaking applications in telepresence, VR and AR.
Most of these methods have focused on static scenes and synthetic data, leaving apart the computational time required, which is still prohibitive.
In contrast, many potential usages of reconstruction and rendering are ideal candidate applications for smartphones, or other consumer-level devices, whose sensors are improving every year but still of limited quality. % and the computational budget.
Our objective is to create a dataset that recreates {\em in the wild} conditions emulating smartphone users.

% Why is it hard?  Real vs synthetic
The SmartPortrait dataset\footnote{https://MobileRoboticsSkoltech.github.io/SmartPortraits/}  is an effort to bridge the gap between realistic raw data obtained from people, collected from a handheld smartphone and the down-stream reconstruction applications, for instance 3D portrait  reconstruction,  view  synthesis,  etc.
The key component that links both views is camera pose {\em state estimation}.
%This problem is usually obviated if working with synthetic high-resolution \cite{s with this} models, at the cost of loosing some realism.
A usual practice is to obtain these poses by using a reliable but computationally demanding Structure from Motion (SfM) algorithm such as COLMAP \cite{schoenberger2016sfm} or multi-modal SLAM methods \cite{campos2021orb,openvslam2019,leuteneger2014okvis,Rosinol20icra-Kimera}.
The trajectories provided in our dataset emulate handheld movements, as if the user, or close-by users, were recording the sequences (see Fig.~\ref{fig:teaser}).


% hard 2: static vs dynamics
Many view synthesis methods \cite{mildenhall2020nerf,gao2020portrait,park2021nerfies,sevastopolsky2020relightable} generate their own datasets just by using state estimation methods. These single camera free-viewpoint images can only be considered if the scene is {\em static.}
%At the same time, there exists a major challenge that has not been untapped to its full magnitude: dynamics. 
% why is it important. Smartphone data generated description
%The data we generate recreates a handheld smartphone video.
We asked volunteers to stay as still as they could while recording them in a semicircular trajectory from close and mid distances.
We observed that most of the volunteers slightly changed their postures so we should expect some degree of displacement, which transforms the problem into {\em non-static}.

%A stream of data where the principle object is a person (non-static), adds all sorts of problems that need to be properly addressed.
The SmartPortrait dataset is obtained in a variety of emplacements,  under different lightning conditions, plus a flashing light from the smartphone at regular intervals.
The smartphone camera is complemented with a high-quality depth sensor, adding robustness and multi-modality. % to the system.

% What do we do?
We provide a recorded dataset consisting of smartphone video images,  IMU data, perfectly time aligned, and an external depth camera from Azure Kinect DK.
The evaluation includes two steps: first we compare the most promising methods with a reference trajectory obtained from a motion capture (MoCap) system. Second, for some environments, it is not possible to deploy the MoCap system. Therefore, we provide a reference trajectory, obtained from the previous best performing method, and provide an upper bound of the error by using a non-reference metric \cite{kornilova2021mom}.
In further evaluations, 
we benchmark multiple state of the art methods for visual SLAM, SfM and Visual-Inertial based methods.

Next, we want to connect the problem of camera pose estimation with two downstream tasks: 3D reconstruction with COLMAP~\cite{schoenberger2016mvs}, ACMP~\cite{xu2018monoperfcap} and SOTA view synthesis algorithms (NeRF \cite{mildenhall2020nerf}, FVS~\cite{Riegler2020FVS}, SVS~\cite{riegler2021stable}).
These applications will help us to understand the importance of pose estimation and its correlation with other tasks.


% The ground truth provided is taken from stereo ORB-SLAM \cite{}, which requires extensive computational time.
% Our advantages
% \begin{itemize}
%     \item Real large sample set (200 people, 5 tracks for every person)
%     \item Smartphone data perfect for VIO algorithms: camera and IMU (accelerometer/gyro)
%     \item Diversity of persons (man/woman, glasses, beard)
%     \item High-quality depth data synchronized with a smartphone (Azure Kinect)
%     \item Lightning. Where it is necessary? - normal estimation, albedo
% \end{itemize}



% In what tasks this data could be used?

% \begin{itemize}
%     \item Training models multi-view rendering with relighting effect
%     \item 3D reconstruction from monocular camera
%     \item Smartphone visual-inertial odometry on real-life data
%     \item Depth prediction from 1 shot
% \end{itemize}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.99\textwidth]{images/Views.pdf}
%   \caption{Show continuity of the trajectory}
%   \label{fig:views}
% \end{figure*}

{\bf Ethical considerations.} We asked all participants in the dataset for a signed consent to record their portraits and publicly release them for  purely academic purposes. We explicitly indicated in the agreement their right, at any time, of removing all their data.
%The purpose of the data is purely academic. 
%The personal data provided is an extremely sensitive issue, and although participants gave their consent, any incorrect use of the data could result 

==> CVPR'21 Avatar dataset (Camera Ready)/src/02_related.tex <==
\section{Related work}
\label{sec:related}

%\subsection{Human Datasets}

Capturing human data is always addressed to a particular task, for instance, human faces, portraits, facial expressions, hand gestures, full bodies, etc. The common trait is that obtaining these data is a challenging process and different approaches exists to tackle them.
Our data include human portraits, or upper body of people, and there exists a relation to many other works on capturing human data. This section reviews the existing literature based on the sensor set used to obtain them. Later, we will discuss some applications and finally, we will present some state estimation methods as a requirement for single free-viewpoint recordings.

% Mocap as multicamera v1.1
{\bf Motion Capture} systems \cite{vicon,optitrack} utilize multiple customized cameras to accurately detect reflective or infra-red markers. They are a popular method used to capture human data by tracking markers and synchronize them with video: HumanEva \cite{sigal2010humaneva}, Human3.6M \cite{ionescu2013human3} and INRIA \cite{Jinlong2016inria}. A negative effect is that it requires the volunteers to wear special suites over their bodies, changing their clothing appearance.

% Multi-camera
{\bf Multiple cameras} overcome this issue and remove the need for {\em markers}. They are a very popular method to capture body expressions and fine details, preserving visual appearance of the models.
Examples include
shape capture \cite{vlasic2009dynamic},
streamable free-viewpoint \cite{collet2015high},
AIST \cite{tsuchida2019aist},
Panoptic studio \cite{joo2017panoptic, joo2018total} with a mixture of  500 cameras, BUFF \cite{zhang2017detailed} for human pose and shape estimation, 
Humbi \cite{yu2020humbi} for body expressions, \cite{gao2020portrait, wang2021learning} for head portraits,
or photo-realistic full-body avatars \cite{bagautdinov2021driving}.
These settings are in practice very precise at capturing simultaneously the same event, e.g. a dynamic person. They are however expensive, difficult to deploy in different environments, and require a considerable amount of effort to calibrate and synchronize them.




% Lightnng variants
Controlled {\bf lightning} conditions are also becoming an important feature for obtaining a fine detailed geometry reconstruction when digitizing humans \cite{vlasic2009dynamic,guo2019relightables, sevastopolsky2020relightable}.
SmartPortraits includes some images under smartphone flash conditions,
%, on its equivalent in a portable smartphone device, %Gnzalo: I removed this, makes no sense
such that the  lightning source coincides with the optical sensor frame and creates a different outcome than under ambient lightning.

% lowere requirements Depth
Some attempts have tried to lower the demanding requirements of multi-camera settings, where many sensors and lightning sources are required.
One solution is enhancing the data obtained with a single {\bf depth sensor} \cite{li20133d, shapiro2014rapid, bogo2015detailed, yu2018doublefusion, guo2017real} or multiple depth sensors \cite{zhang2012real, dou2016fusion4d, hong2018dynamic}.
%maybe IMU + cameras?
% Sparse cameras
Other approaches try to reduce the number of cameras in operation and still obtain reasonably accurate results \cite{zheng2021deepmulticap, zhang2021lightweight}.


% stereo

% Single camera
At the extreme, one would desire a {\bf single camera} free-viewpoint, either taking multiple pictures or with a video \cite{xu2018monoperfcap, alldieck2019learning}. This is the aim of our dataset as well.





\begin{table*}
%\tiny%small
\fontsize{7.9}{7.2}\selectfont
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\bgroup
\def\arraystretch{1.5}%
\begin{tabular}{p{0.079\textwidth}p{0.136\textwidth}p{0.114\textwidth}p{0.114\textwidth}p{0.202\textwidth}p{0.114\textwidth}p{0.114\textwidth}p{0.128\textwidth}}
\toprule
 & EuRoC MAV & TUM-VI & TUM RGB-D & PennCOSYVIO & KAIST VIO & ADVIO & Ours \\
\midrule
Year & 2016 & 2018 & 2012 & 2016 & 2021 & 2018 & 2021  \\
Environ- ment & indoors & indoors/ \newline outdoors & indoors & indoors/ \newline outdoors & indoors & indoors/ \newline outdoors & indoors \\
Carrier & MAV & handheld & handheld/robot  & handheld & UAV & handheld & handheld \\

Focus & MAV VIO/SLAM & VIO & RGB-D SLAM & handheld VIO & UAV VIO & handheld VIO/SLAM & VIO/SLAM in\newline Human Digitiz.  \\

Cameras & 
stereo gray: 2x752x480 @20Hz &
stereo gray: 2x1024x1024 @20Hz &
RGB-D: \newline 640x480 @30Hz &
\textbullet\ 4 RGB: 1920x1080 @30Hz \newline
\textbullet\ stereo gray: 2x752x480 @20Hz \newline
\textbullet\ fisheye gray: 640x480 @30Hz &
\textbullet\ RGB: 640x480 @30Hz \newline
\textbullet\ stereo IR: 640x480 @30Hz&
\textbullet\ RGB: 1280×720 @60Hz \newline
\textbullet\ fisheye gray: 640x480 @60Hz &
\textbullet\ RGB: 1920x1080 @30Hz \newline
\textbullet\ depth: 640x576 @5Hz \\

IMUs &
ADIS16448 3-axis acc/gyro @200Hz &
BMI160 3-axis acc/gyro @200Hz &
Kinect 3-axis acc \newline @500Hz &
\textbullet\ ADIS16488 3-axis acc/gyro @200Hz \newline
\textbullet\ Tango 2 3-axis acc @128Hz \newline
\textbullet\ Tango 2 3-axis gyro @100Hz & 
Pixhawk 4 Mini 3-axis acc/gyro @100Hz &
MP67B 3-axis acc/gyro @100Hz &
\textbullet\ LSM6DSO 3-axis acc/gyro @500Hz \newline \textbullet\ MPU-9150 3-axis acc/gyro @500Hz\\

Time sync & hw & hw & hw & hw, sw & data & sw & hw, sw + frame sync \\
Point clouds & \checkmark (some seq) & $\times$ & \checkmark & $\times$ & $\times$ & \checkmark & \checkmark \\

Distance &
11 seq, 0.9 km &
28 seq, 20 km &
39 seq x several m &
4 seq, 0.6 km &
14 seq x several m &
23 seq, 4.5 km &
1000 seq, 6.6km \\
\midrule

Ground-truth & 
\textbullet\ 3D pos. (some seq), laser tracker @20Hz \newline
\textbullet\ 3D pose (some seq), MoCap @100Hz \newline
\textbullet\ 3D pcds (some seq), laser tracker & 
3D pose, MoCap @120Hz \newline (partial gt) & 
\textbullet\ 3D pose, MoCap @300Hz (partial gt) \newline
\textbullet\ 3D pcds, Kinect @5Hz & 
3D pose, visual markers @30Hz &
3D pose, MoCap @50Hz &
\textbullet\ 3D pose, IMU + manual position fixes @100Hz \newline
\textbullet\ 3D pcds, Tango @5Hz&
\textbullet\ 3D pose (some seq), MoCap @240Hz \newline
\textbullet\ 3D pose, COLMAP/RGB-D SLAM @5Hz \\

Acc. $\approx$ &
1 mm &
1 mm (static case) &
1 mm (relative) &
15 cm &
1 mm & 
0.1 - 1 m \cite{wang2019near} & 1 mm - 1 cm \\

\bottomrule
\end{tabular}
\egroup
} % \resizebox
\caption{Overview of common Visual (V) and Visual Inertial (VI) benchmark datasets targeted at state estimation. 
%Marsel I would put "...common V/VI benchmark..." Yes
}
\label{tab:related}
\label{tab:datasets_vo_vio_slam}
\end{table*}


From the perspective of datasets capturing human data for people reconstruction and rendering task, we observe the following modelling classes: full body modelling (DynamicFAUST~\cite{bogo2017dynamic}, BUFF~\cite{zhang2017detailed}, People Snapshot~\cite{alldieck2018video}), clothes modelling (3DPeople~\cite{pumarola20193dpeople}, SIZER~\cite{tiwari2020sizer}), \textit{head/torso portrait} modelling (UHDB11~\cite{toderici2013uhdb11}, Nerfies~\cite{park2021nerfies}, Portrait Neural Radiance~\cite{park2021nerfies}), or suitable for applications in couple of tasks (RenderPeople, Humbi~\cite{yu2020humbi}). There are also crowd-sourced datasets such as MannequinChallenge~\cite{li2019learning}, TikTok Dataset~\cite{jafarian2021learning} collected from social networks available for reconstruction tasks. Our dataset is unique since it records consumer-level data (smartphone) ``in the wild'' supported by high-quality external depth data.

Recently emerged neural implicit representation methods allow to bypass the need for obtaining accurate 3D structure of a scene and instead model it implicitly, e.g. by considering occupancy \cite{mescheder2019occupancy}, signed distance function \cite{park2019deepsdf} or volumetric density \cite{mildenhall2020nerf,  lombardi2019neuralvolumes}. In particular, there have been several works that successfully used neural implicit representation for creating realistic portrait avatars \cite{gao2020portrait, park2021nerfies, wang2021learning, gafni2021dynamic, sevastopolsky2020relightable}.

% If the scenes are static, then it is possible to use create multiples views from a single camera. A recently neural implicit representation 
% \gf{konstantin, I need you now to put all these methods into here}
% Groundbreaking methods on image synthesis \cite{mildenhall2020nerf, mildenhall2019local},
% reconstruction \cite{},
% collect their own dataset, as a set of images for which later state estimation techniques for camera poses are used. COLMAP \cite{schoenberger2016sfm}

%single camera adapting to dynamics?

Unfortunately, when scenes include dynamic elements, and that is the case of video recording of people, the state estimation of camera poses or free-viewpoints and the 3D scene is not so trivial.
In the downstream tasks of 3D human reconstruction, two main variants exist:
free-form \cite{carranza2003free,saito2019pifu,saito2020pifuhd}
and model based \cite{loper2015smpl,alldieck2018video,omran2018neural}. 


%\subsection{Visual SLAM Datasets}
% -----------------------------------------------------------------
% Linking with human recording and SLAM
% -----------------------------------------------------------------


Accordingly, when reducing the number of cameras to a single one and working in {\em non-static} conditions because the volunteers in our dataset stand still but not immobile, then,
{\bf state estimation} becomes the key ingredient that allows a handheld single camera video to be used for human digitization.
Either if camera poses are compensated while learning a model \cite{lin2021barf} or estimated as recorded, the quality of these is going to be determinant for any downstream task.






To the best of our knowledge, there are no datasets that directly address the evaluation of state estimation approaches when a human is in the main focus of sensors.
State estimation of camera poses include techniques such as 
Visual Odometry (VO) \cite{Forster2014ICRA,DBLP:journals/corr/EngelKC16},
Visual-Inertial Odometry (VIO) \cite{leuteneger2014okvis,qin2019local,PRCV-LiYHZB2019,bloesch2017rovio}. Variants of Simultaneous Localization and Mapping (SLAM), which include a loop in estimation for global pose alignment, either 
Visual SLAM  (V-SLAM) 
\cite{mur2015orb,gao2018ldso,mur2017orb,openvslam2019} or 
Visual-Inertial SLAM (VI-SLAM)
\cite{qin2017vins,Rosinol20icra-Kimera,Geneva2020ICRA,campos2021orb} and Structure from Motion (SfM) \cite{schoenberger2016sfm}, all of them relevant to the be applied to the sensor data available in a smartphone.
To date, there are numerous datasets available \cite{Burri25012016, jeon2021run, tumvi, sturm12iros, penncos, Cortes_2018_ECCV, geiger2013vision, Delmerico2019drone, carlevaris2016university, ceriani2009rawseeds, zuniga2020vi, wang2019near} that vary greatly by their focus, recording environment, sensor carriers as well as by the amount of data recorded and the accuracy of the ground truth.
%Due to this, we choose the datasets that are the most related to our work based on their setups. 
We briefly describe the main features of the main datasets and give a comparison with our dataset (see Table \ref{tab:related}).

The EuRoC Micro Aerial Vehicles (MAV) dataset~\cite{Burri25012016} focuses on VIO and SLAM for MAVs as well as 3D reconstruction. 
The authors employ a stereo pair of cameras hardware-synchronized with an IMU installed on a MAV for acquiring the data sequences in two indoor environments. %: a large industrial machine hall and a room. 
%Ground-truth data for sequences are of high precision, however, 6D poses, as well as point clouds, are available only for the sequences captured in the room.
Kaist VIO \cite{jeon2021run} is another indoor dataset that focuses on VIO for aerial vehicles, it specifically addresses challenging scenarios for VIO that contain pure rotational/harsh motions. %Unlike EuRoC MAV, Kaist VIO provides accurate 6D ground-truth poses acquired with motion capture system (MoCap) for all sequences.
TUM-VI \cite{tumvi} is a dataset for the purpose of evaluating VIO algorithms. Compared to other mentioned datasets it stands out by its size, diversity of the recorded sequences, as well as uses higher resolution cameras. %Trajectories of some sequences go out of places with installed MoCap system, so accurate ground-truth data are provided only for the beginning and the ending parts of such sequences.
TUM RGB-D \cite{sturm12iros} features only indoor sequences captured with a Kinect sensor that is handheld or mounted on a robotic platform. The dataset includes challenging scenarios for the proper evaluation of RGB-D SLAM  approaches. %Like in TUM-VI dataset for some sequences the ground truth is only provided at the beginning and the end.
PennCOSYVIO \cite{penncos} is one more VIO benchmark that contains diverse challenging sequences. It includes not only rotational motions but hard visual conditions as well. The dataset was captured using a larger number of sensors than any other related datasets: 3 GoPro cameras, an integrated VI-sensor and 2 Google Project Tango tablets mounted on a rig. However, as pointed out in \cite{tumvi} the setup yields lower synchronization accuracy between cameras and IMUs when compared to datasets like TUM-VI. %For acquiring the ground truth the authors used AprilTags placed along the route of recording as the environment didn't allow for using more precise measurement tools. The ground truth was verified by capturing additional sequences at different places for which more precise ground truth was known.
ADVIO \cite{Cortes_2018_ECCV} focuses on benchmark VIO and SLAM methods for smartphones and mobile devices with low-cost sensors. It contains different large indoor and outdoor environments recorded in public places. %The ground truth is collected using a method proposed by the authors that is designed for such environments where the use of visual markers, motion capture or laser scanners is not possible. The authors do not report the estimated accuracy of the gathered ground-truth poses.

Our dataset contains recordings of people in indoor environments and focuses on the diversity of people, their clothing, the environments and the lightning conditions, totally uncontrolled aiming to recreate every-day life conditions of smartphone users.
%\gf{what is the high quality sensor?? I removed this because it is not high quality to my standards}
%We use a combination of low-cost and high-quality sensors for gathering the data (see section \ref{sec:system_design}).
Compared to PennCOSYVIO, KAIST VIO and ADVIO that use heterogeneous sensors too, we employ a significantly more precise hybrid hw/sw synchronization technique from \cite{faizullin2021synchronized} (see Sec.~\ref{sec:sys_sync}).
Due to recordings surroundings peculiarities we provide pseudo-ground truth poses based on the gathered sensors data like in \cite{Cortes_2018_ECCV} the quality of whose is estimated in a manner similar to \cite{penncos} by capturing verification sequences (see Sec.~\ref{sec:gt}).


% We need to move missing citations to above.
%We considered to run our dataset on the most well-know Visual Odometry (VO), and Visual Inertial Odometry methods, to evaluate and compare the final estimated trajectory results. These methods are known as: OpenVSLAM (A Versatile Visual SLAM Framework)\cite{openvslam2019}, LDSO (Direct Sparse Odometry with Loop Closure)\cite{DBLP:journals/corr/abs-1808-01111} and ORB-SLAM3 Monocular (An Accurate Open-Source Library for Visual, Visual-Inertial and Multi-Map SLAM)\cite{ORBSLAM3_2020} for VO category. And furthermore, ORB SLAM Monocular-Inertial\cite{ORBSLAM3_2020}, Kimera VIO (an Open-Source Library for Real-Time Metric-Semantic Localization and Mapping)\cite{Rosinol20icra-Kimera}, OpenVINS (houses some core computer vision code along with a state-of-the art filter-based visual-inertial estimator)\cite{Geneva2020ICRA}, VINS-Fusion (an optimization-based multi-sensor state estimator, which achieves accurate self-localization for autonomous applications)\cite{qin2019a}\cite{qin2019b},    VINS-Mono (a real-time SLAM framework for Monocular Visual-Inertial Systems)\cite{qin2017vins}, PVIO (Robust and Efficient Visual-Inertial Odometry with Multi-plane Priors)\cite{PRCV-LiYHZB2019}, OKVIS (Open Keyframe-based Visual-Inertial SLAM)\cite{article} and ROVIO (Iterated extended Kalman filter based visual-inertial odometry using direct photometric feedback )\cite{doi:10.1177/0278364917728574}, are implemented for VIO methods. 








==> CVPR'21 Avatar dataset (Camera Ready)/src/03_system_design.tex <==
\section{Recording Platform}
\label{sec:sys}

Our dataset aims to provide human portrait data in the realistic environments captured by a middle-price smartphone. To meet these requirements, we have designed a portable handheld platform with a \textbf{Samsung S10e} smartphone (RGB camera, 1920x1080 p, 30 fps; IMU, 500 Hz, flasher, 1 Hz) and a high-end depth sensor \textbf{Azure Kinect DK} (depth camera, 640x576 p, 5 fps).  The high-quality external depth camera is chosen instead of the smartphone with a built-in sensor as (i) the modern smartphone depth images are still not as high-quality as external depth sensors, and (ii) it is not possible to record RGB and depth tracks by the smartphone on high frequency simultaneously. A common view of the system is presented in Fig.~\ref{fig:system_common_view}. 

%The independence of smartphone and depth camera adds an additional challenge to the time synchronization during the recording that we solve as described in Sec.~\ref{sec:sys_sync}.
%Details on extrinsics and intrinsics calibration parameters for our platform are discussed in Sec.~\ref{sec:sys_calib}. 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{images/common_view2_50.jpg}
  \caption{Front and back view of the recording platform. }
  \label{fig:system_common_view}
\end{figure}


Specifics of our recording case~--- dynamic camera movements close to real-life handheld capture and a person in foreground with non-stationary pose (blinking eyes, small movements of the person because of breath, coordination, heart beats). 

%These details arise additional requirements for sync quality between depth and smartphone camera, because if frames from both sensors captured at slightly different time, they could not accurately correspond and create artifacts during data fusion for SLAM or reconstruction applications and leads to incorrect depth correspondences or other artifacts.


\subsection{Time and Frame Synchronization}
\label{sec:sys_sync}


%The synchronization of capturing frames from smartphone and depth cameras of our system is a two-step process. 
The independence of smartphone and depth camera adds an additional challenge to the time synchronization. If frames from both sensors are captured at slightly different instants of time, several tens of $ms$, this degrades the quality of the camera pose estimation.

To synchronize the cameras, we introduce a two-step sync process.
First, the time domains between two sensors are synchronized by Twist-n-Sync algorithm~\cite{faizullin2021twist} which is not affected by network asymmetry, in contrast to network-based protocols like NTP. And in the second step~-- the synchronization of frame capturing moments from both sensors is done. For solving that, the grabbing of the smartphone's framing phase is performed via remote API interface. Then depth camera triggering is automatically tuned to this phase as explained in~\cite{faizullin2021synchronized}.
The sync used provides sub-millisecond accuracy.
%For that we start record on the smartphone, obtain its phase parameters via remote API interface and adopt depth triggering to this phase in common time domain.

%\subsection{Design solutions}
%\label{sec:system_design}
 
%\gf{if we remove this part, the content remains unchanged. WHy? we record images in some format, regardless of what we used}   
%\textbf{Hardware} For launching synchronous data capturing, additional hardware has been/is used: mini PC, MCU( microcontroller unit)-board, standalone IMU that together share tasks on recording and synchronization. Complete description of the platform's parts and their tasks can be found in~\cite{faizullin2021synchronized}.


%\textbf{Software} The platform software consists of two main components~--- (i) ROS-based software that is ran on the mini PC and (ii) OpenCamera Sensors~\cite{opencamsensors} application that is ran on the smartphone. ROS-based software is the main entry point in the data collection process~--- it controls the start and stop of the recording, triggers depth frames capturing via MCU board, interacts with the smartphone over Wi-Fi for synchronization of smartphone camera and depth streams. The system configuration allows us to start and stop the recording process via SSH independently from the operator that carries the platform. Data collection on the smartphone is performed via OpenCamera Sensors application, which supports remote control interface via the network, provides synchronization of smartphone camera and IMU sensors, and shares information about camera phase parameters for synchronous frame capturing with depth.

\subsection{Calibration}
\label{sec:sys_calib}

%Since we provide data from imperfect sensors that differently placed on a metal rig, intrinsic and extrinsic calibration must be applied to them. 
The full intrinsic and extrinsic calibration of smartphone camera and smartphone IMU, is obtained by the Kalibr toolbox~\cite{rehder2016extending} with 6x6 AprilGrid array of 3x3 cm AprilTags~\cite{olson2011apriltag} as the visual markers. 

%Intrinsic calibration of depth camera is not carried out since it is factory calibrated and the parameters are provided out-of-the-box. 
%\gf{this needs more active and positive sentences, say what we do and not what we cant} 
%Because of pure quality of depth camera infra-red images, direct depth-to-smartphone camera transformation cannot be obtained by Kalibr. 

To find depth-to-smartphone camera transformation, firstly, we obtained the Azure RGB to smartphone camera transform. Then, combined it with the factory-known Azure depth (infra-red) to Azure RGB camera transform. This method gives much better accuracy than direct depth-to-smartphone camera transformation with low-quality infra-red camera. We use Azure RGB only for this procedure. All the obtained transformations are shown in~Fig.\ref{fig:transforms}.

Smartphone camera is rolling-shutter type; however, we applied global-shutter camera model during calibration to feed the calibration parameters correctly to the methods we compared in Sec.~\ref{sec:eval}. 
%Furthermore, Standalone IMU calibration is also performed. Instead of generating data and analyzing Allan plots to obtain IMUs noise parameters, we acquired them from~\cite{lsm6dso} and~\cite{nikolic2016non} for smartphone and standalone IMU respectively.
Standalone IMU calibration is also performed. IMUs noise parameters were borrowed from~\cite{lsm6dso} and~\cite{nikolic2016non} for smartphone and standalone IMU respectively.

%!\mf{somewhere mention about transformation obtaining by optimization}
%OK\mf{add visual marker params}
%OK\mf{edit image with transforms}
%OK\mf{about allan}
%OK\mf{intrinsics}
%OK\mf{6D pose}
%OK\mf{azure smartphone}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{images/transforms.png}
  \caption{Obtained relative transformations by calibration. $^I T_C$~-- smartphone camera in smartphone IMU reference frame, $^C T_D$~-- depth camera in smartphone camera frame. $^C T_D$ is found as $^C T_D = ^C T_R \cdot ^R T_D$, where $^C T_R$ is Azure RGB camera in smartphone camera frame obtained by Kalibr, $^R T_D$ is factory-known Azure RGB camera in Azure depth camera frame. Azure RGB is only used for this procedure.}
  \label{fig:transforms}
\end{figure}


% \ak{From Konstantin, but let's describe last exp}
% In order to find intrinsic parameters and to amend for the distortions of the cameras, we perform a calibration procedure. We use a $8 \times 6$ chessboard calibration pattern with a square size of 55 mm and calibration utilities provided by OpenCV \cite{2015opencv} that are based on the method described in \cite{zhang2000flexible} to determine the required parameters. They are focal length, optical center, and 8 distortion coefficients. We have chosen a rational distortion model with 8 coefficients because of the poor performance of the 5-coefficient model. We explain it by the huge geometric imperfection of smartphone camera lenses.


%\subsubsection{Smartphone Camera to Depth Camera Calibration}
\label{sec:calib_cam2depth}

%\mf{still have hole in explanation of kalibr vs. opencv calib of cameras}\\
%\mf{Shorten if possible}

%To get relative transformation between depth and smartphone cameras, we employ the following procedure. 

%Firstly, we detect chessboard calibration pattern corners by both cameras. 
%\mf{Explain if you are about gray images of depth camera, here is no exact statement} Next, we estimate the poses of the detected corners in the local system of coordinates for each camera. For depth camera, to translate keypoints from the image plane to the local camera coordinates, we use provided depth measurements, whereas for smartphone camera we solve the PnP problem using IPPE \cite{collins2014infinitesimal} implemented in OpenCV \cite{2015opencv}. Then, we estimate the initial transformation between two point clouds of chessboard corners using the method described in \cite{horn1988closed}. We have found that it gives a slightly more accurate initial guess than \cite{arun1987least} due to the planarity of two sets of points. The obtained initial guess is usually very coarse due to the significant difference in the intrinsic parameters of the cameras. Thus, to ensure that the transformation correctly maps keypoints between images recorded by both cameras, we further refine the parameters of the initial transformation subject to epipolar constraints between the keypoints using \mf{open abbreviation}LM. As epipolar constraints influence only the direction of the relative translation between cameras poses, we additionally perform a line search along the direction to acquire the magnitude. The final transformation is produced by averaging several refined estimates where the recorded calibration pattern is stationed at different distances from the cameras.
%\gf{I agree, we use a standard technique plus epipolar refinement, one paragraph should enough}


==> CVPR'21 Avatar dataset (Camera Ready)/src/04_dataset.tex <==
\section{Dataset}

Our dataset contains 1000 records of 200 people, with natural clothing, captured in different native locations and poses. Every record consists of synchronized smartphone data (Full HD RGB video, flash timestamps, timestamped accelerometer and gyroscope measurements) and the depth images from external high-quality depth sensor. The dataset also contains reference ground truth trajectories of the smartphone camera obtained as described in Sec.~\ref{sec:gt} and segmentation masks for the person.
We supplement the dataset by labels for genders and difficult cases for rendering like volume hairs/beard/glasses.
Data parameters and sampling rates of the sensors are presented in Table.~\ref{tab:datasets_vo_vio_slam}.
%This section describes the data collection process, collected statistics, person masks generation procedures.


\subsection{Collection Process and Statistics}


During every recording process, three people are involved: 
(1) a volunteer who is being filmed, (2) an operator that carries the recording platform, and (3) an assistant that monitors the correctness of the recording through SSH.
The volunteer is asked to stand or sit still. The operator carries a recording platform around the person at the subject's face height as depicted in Fig.~\ref{fig:teaser}. 
The recording trajectory begins in front of the person to capture the whole scene, then the operator moves to a side of the volunteer and makes four 100-120 degrees circular arcs around the model. The entire trajectory is shown in Fig.~\ref{fig:teaser}. 
The timestamps of every arc edge are marked online during recording by the assistant in an automated manner. In post-processing  stage, the whole trajectory could be split into separate arcs applying these marks.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/Recording.pdf}
%   \caption{Show recording process}
%   \label{fig:recording_process}
% \end{figure}

Every person is captured in 5 different poses~--- 3 in a standing position (straight, hand on hips, with head turned) and 2 in a sitting position (straight, with head turned). %, as depicted in Fig.~\ref{fig:recording_poses}. 
Standing and sitting positions were captured from a distance of about 2 and 1 m respectively. 
During the recording, blinking flash on the smartphone is turned on with a frequency of 1 Hz to relight the model. Effect of re-lightning is more distinguishable on sitting positions since they are captured from a closer distance.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/Relightning.pdf}
%   \caption{Demonstration of re-lightning effect by the smartphone flash that is used during recording at 1 Hz frequency. {\em Left:} Ambient illumination. {\em Right:} Illumination with flash.}
%   \label{fig:relightning}
% \end{figure}

Data collection is performed in 5 different locations of native indoor environments: cafeteria, lab, office, campus entrance, and student council. Their common view is demonstrated in Fig.~\ref{fig:teaser}. 
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/Poses.pdf}
%   \caption{Show poses}
%   \label{fig:recording_poses}
% \end{figure*}
The average length of the trajectories for staying and sitting position are 7.14 and 5.8 m accordingly. The total duration of all tracks is 11 hours and 6 minutes, and the total length is 6610 meters.


SmartPortrait contains people of different gender, appearance, clothing, hairstyles, etc. Statistics are shown in Fig.~\ref{fig:dataset_stat}.

%Since 3D reconstruction and rendering of humans are complicated on the parts with glasses and hairs (beard, voluminous hairstyles), we also added labels for this; 


\begin{figure}[t]
  \centering
   \includegraphics[width=0.95\linewidth]{images/DataStat2-2.pdf}
  \caption{Dataset statistics. {\em Left:} Locations of recording. 
  %Marsel remove "of recording"
  {\em Center:} Gender {\em Right:} Appearance.}
  \label{fig:dataset_stat}
\end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/mask_pipeline.pdf}
%   \caption{Semi-automated pipeline for human mask segmentation. {\em Top-Left:} Original frame from the dataset video. {\em Top-Right:} Mask generated by U2-Net~\cite{qin2020u2} pre-trained on person datasets. {\em Bottom-Left:} DBSCAN clustering of mask using information from depth camera (white and red are different clusters). {\em Bottom-Right:} Corrected mask.}
%   \label{fig:dataset_masks}
% \end{figure}


\subsection{Segmentation Masks}

Along with recorded data, we also provide segmentation masks of humans on the images. This information could be used for filtering out potentially dynamic landmarks of the scene on the trajectory estimation step (blinking eyes, subject movements) as demonstrated in Sec.~\ref{sec:gt} or for separation of portraits parts from the scene for only-person 3D reconstruction.
For this task, we design a semi-automated labeling process, based on U2-Net~\cite{qin2020u2} that is pre-trained on people masks from the Supervisely Person Dataset~\cite{supervisely}. Usage of this method on our data overestimates the person mask, also covering some parts of the background. DBSCAN clusters the masked part by using the depth component, discarding scene parts that are not related to the foreground. Finally, segmentation results are assessed visually by labelers.




==> CVPR'21 Avatar dataset (Camera Ready)/src/05_evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{images/mocap-eval-newmetric.pdf}
  \caption{Full-reference (APE/RPE) and no-reference (MOM) metric statistics for COLMAP and ORB SLAM (RGB-D) for 5 test sequences with MoCap ground truth poses. (b) and (p) indicate that only background keypoints and person keypoints correspondingly were considered for pose estimation. One pose for ORB SLAM (p) is not converged, therefore its values are excluded from the evaluation.}
  \label{fig:mocap_eval}
\end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{images/vi-eval-all-newmetric.pdf}
  \caption{Evaluation of V/VI methods that employ only smartphone data (frames and IMU) on benchmark sequences.}
  \label{fig:vi-eval}
\end{figure*}

The evaluation part tackles two main questions~--- (1) how to find the best way of calculating pseudo-ground truth poses for our dataset and (2) investigate the performance of V and VI state estimation methods on smartphone data only.
V denotes all visual methods: VO and V-SLAM; the same applies for VI.

\subsection{Metrics}

\textbf{Full-reference metrics.} Among the class of full-reference metrics where the reference trajectory (ground truth) is available, we consider RMSE statistics on Absolute Pose Error (APE) and Relative Pose Error (RPE) for the rotation and translation parts. In particular, for translation APE, we apply the Umeyama alignment~\cite{arun1987least,umeyama1991} between a pair of trajectories if expressed in different origin frames. For rotation APE, the Umeyama alignment is followed by the trajectory's reference frame transformation.

\textbf{No-reference metrics.} No-reference metrics are alternative to the full-reference metrics when the reference trajectory is not available or its quality is disputable. In our work, we use Mutually Orthogonal Metric (MOM)~\cite{kornilova2021mom} that measures quality of the trajectory by evaluating quality of the map aggregated from point clouds registered via the trajectory poses. MOM provides stronger correlation with RPE error in comparison to its competitors~\cite{razlaw2015evaluation}. In our setting, MOM uses the point clouds converted from depth images.


In order to apply MOM on trajectories ambiguous to scale (e.g., COLMAP), we optimize the scale factor w.r.t. MOM metric~---  which assumes that the correct value of scale is reached at the optimum in the metric, when the aggregated map of point clouds is at its best condition.

\subsection{Ground Truth Trajectories}
\label{sec:gt}

The majority of the dataset sequences (see Fig. \ref{fig:dataset_stat}) are captured in public places or areas where either applying conventional methods of acquiring ground-truth poses (e.g., MoCap) are not feasible, or such methods disrupt the nativity of the surroundings (e.g., visual markers).

%Marsel Therefore, a no-reference method is required 
Therefore, it is required a no-reference method in order to validate the obtained trajectories when MoCap data is not available. Below, we will present a procedure to select a new reference trajectory and an upper bound of its error.


% Hence following \cite{} we provide pseudo-ground truth poses (referred to as ground truth next in the text) that are calculated based on the collected sensors data. \ak{Which one do we provide?}

\textbf{Methods.} Since the dataset is targeted on both state estimation and reconstruction/synthesis domains, we consider the main methods typically used by the community that make use of the sensors: RGB, depth cameras and IMU.
From \textit{reconstruction and rendering} field experience, we consider the COLMAP \cite{schoenberger2016sfm} Structure-from-Motion (SfM) pipeline that is de-facto standard tool in this area and usually employed as ground truth. COLMAP uses only RGB data and therefore its trajectory is defined up to a scale factor, that limits its usage in state estimation tasks. In addition, we consider the class of RGB-D SLAM algorithms that are able to provide poses and scale is observable.
%and it is more stable than other state estimation methods that doesn't use depth data~\ak{cite, proof} \gf{last statement requires citation, if not remove} \mf{agree}. 
Based on the wide evaluation of RGB-D SLAM methods done in~\cite{zhang2021survey} we choose ORB-SLAM (RGB-D) \cite{mur2017orb}, implementation from \cite{campos2021orb}, as one with the lowest trajectory error.
%Marsel Actually, if I am not mistaken, we used ORB-SLAM 3 \cite{campos2021orb} 

\textbf{MoCap Test Sequences.} To assess the accuracy of the ground truth poses, we record several testing sequences in the laboratory environment where the use of a more accurate ground truth acquisition method is possible. In particular, we utilize OptiTrack MoCap system \cite{optitrack} to record 5 testing sequences of one person in the common dataset format. MoCap is synchronized with the platform offline by the Twist-n-Sync algorithm~\cite{faizullin2021twist}. 
The extrinsic parameters calibration requires to calculate:

\begin{equation}
    \min_{X,Y\in SE(3)} \sum_{i} || \log \big( Y \cdot T_M(i) \cdot X \cdot T_C^{-1}(i)\big) ||,
\end{equation}
where $T_M(i)$ is the trajectory given by the MoCap at time $i$, $T_C$ is pose at the camera frame calculated by the algorithm, $X$ is the transformation between the camera optical center and the tracked object in the MoCap and $Y$ is the transformation between the origin frame of the MoCap and the origin of the SLAM algorithm (usually first frame).

\textbf{Results.} In order to support the selection of the pseudo ground truth, we evaluate COLMAP and ORB-SLAM (RGB-D) (actually, virtual stereo) on the MoCap test sequences by using the described above full-reference and no-reference metrics. Because the landmarks on the volunteer body might be non-static (person can breath, blink), we consider three modifications of COLMAP and ORB-SLAM (RGB-D) -- using the whole scene, using mask for background, using mask for person. The evaluation results are presented in the Fig.~\ref{fig:mocap_eval}. Both methods demonstrate almost the same performance on the considered metrics, being close to the resolution limit of the MoCap system. The usage of masks does not affect the performance in case of COLMAP that could be explained by photometric consistency imposed by the algorithm. ORB SLAM performs worse when only part of the scene is visible. 

\textbf{Eval Generalization.} The above evaluation on the MoCap test sequences with ground truth available is limited only to the  lab location. To extend it to all locations that our dataset covers, we must consider the comparison of COLMAP and ORB-SLAM (RGB-D) by  using the no-reference metric MOM. For that, we select 10 trajectories from every location that result into 50 test sequences. Evaluation performance is presented in Fig.~\ref{fig:mom_generalization} and it allows to make the following two conclusions. Firstly, since MOM measures the dispersion of deviations on planar surfaces in the aggregated map it can be noticed that for the majority of locations it does not overcome 2 cm. This value is comparable to the depth sensor noise, that means that both methods give relatively good trajectories from the state estimation point of view. Secondly, COLMAP performs slightly better than ORB-SLAM (RGB-D), although it requires post-processing for revealing the scale. We will provide the obtained trajectories of both methods as the pseudo-ground-truth methods.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{images/MOM-generalization.pdf}
  \caption{MOM generalization to 50 other scenes from the dataset.}
  \label{fig:mom_generalization}
\end{figure}

% It is here because
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{images/ColmapACMP.pdf}
  \caption{Qualitative demonstration of dense reconstruction from different views using COLMAP-MVS (3 left columns) and ACMP (3 right columns) on poses from COLMAP-SfM, ORB-SLAM (RGB-D), ORB-SLAM (V).}
  \label{fig:ColmapACMP}
\end{figure*}


\subsection{V and VI Evaluation}

One of the motivations of our work is the study the potential of applications of V/VI methods using smartphone-only data targeted to the domain of human portraits. In this section, we provide evaluation of different state-of-the-art methods and a baseline for future comparisons. In addition, to all the considered methods, we deliver configuration and calibration files for methods to be used with our data for benchmark.

\textbf{Methods.} In evaluation we consider two classes of methods: Visual (V) and Visual Inertial  (VI) methods. Considering recent exhaustive evaluations~\cite{jeon2021run, delmerico2018benchmark}, we order top-rated V/VI methods. The considered methods for both classes are: for V~--- OpenVSLAM\cite{openvslam2019}, ORB SLAM Monocular\cite{campos2021orb}, LDSO\cite{gao2018ldso} and
COLMAP \cite{schoenberger2016sfm}.
For VI (ordered by performance on other datasets)~-- ORB-SLAM 3 (VI) \cite{campos2021orb}, Kimera VIO\cite{Rosinol20icra-Kimera}, OpenVINS\cite{Geneva2020ICRA}, VINS-Fusion\cite{qin2019local}\cite{qin2019global}, VINS-Mono\cite{qin2017vins}, PVIO\cite{PRCV-LiYHZB2019}, SVO.2\cite{7782863}, MSCKF\cite{4209642}, OKVIS\cite{leuteneger2014okvis}, ROVIO\cite{bloesch2017rovio}. Some of the methods (Kimera VIO, OpenVINS, MSCKF, ROVIO) were discarded because they require recording device to be static over the first seconds of the trajectory for initialization, whereas our use case does not cover such scenario.

\textbf{Benchmark Dataset} To evaluate the performance of the methods, we uniformly pick 2 sequences for every combination of location and volunteer pose, resulting in a total of 50 evaluation sequences. As ground truth, we consider the trajectories produced by ORB-SLAM (RGB-D) that, as demonstrated in Sec.~\ref{sec:gt}, provides excellent performance.

% \textbf{Results.} The evaluation results on the set of the full-reference metrics are presented in Fig.~\ref{fig:vi-eval}. 
% We can observe how V methods perform more accurately in rotation and translation. The VIO method's accuracy varies, where ORB 3 VI performing as accurate as V methods. All VI have better than 1 degree of accuracy in absolute rotation error. 

\textbf{Results.} The evaluation results on the set of the full-reference metrics are presented in Fig.~\ref{fig:vi-eval}. Because the pseudo GT provides a statistical bound, it could be used for exact ordering in cases when the order of the error magnitude is higher than the error between MoCap and pseudo GT. In particular, in our comparison we can order only the next V/VI methods: LDSO, OKVIS, PVIO, SVO2, VINS. In general, we can observe that V methods perform more accurately in rotation and translation than VIO methods. The VIO method's accuracy varies, where ORB 3 VI performing as accurate as V methods. All VI have better than 1 degree of accuracy in absolute rotation error.

==> CVPR'21 Avatar dataset (Camera Ready)/src/06_application.tex <==
\section{Application}
\label{sec:application}

\textbf{3D reconstruction.} For qualitative comparison on 3D reconstruction, we provide poses obtained from the top performing methods for state estimation from every class and use two state-of-the-art methods for 3D reconstruction: COLMAP multi-view stereo (MVS)~\cite{schoenberger2016mvs} and ACMP~\cite{xu2020planar}. The demonstration of the obtained 3D scenes is presented in Fig.~\ref{fig:ColmapACMP} from two views~--- center and the edge of the trajectory arcs. For both reconstruction pipelines, COLMAP trajectory produces less distorted reconstruction, overcoming ORB-SLAM (RGB-D) and (V) versions. It could also be noticed that from the trajectory border point of view 3D reconstruction has less quality.
%that could be explained as \ak{???}.
%Total quality of 3D reconstruction is still not good\ak{say in other words}.
The solution from the VI method produced an incorrect reconstruction, perhaps due to its error.

\textbf{View Synthesis.} We provide a qualitative comparison of the considered VO-SLAM methods evaluated on an image synthesis problem. For that we considered SOTA methods: Neural Radiance Field \cite{mildenhall2020nerf} (NeRF), and generalized NeRF approaches~--- FVS~\cite{Riegler2020FVS} and SVS~\cite{riegler2021stable} in their default pre-trained versions. The data provided to methods is the solution of the trajectories. For NeRF algorithm, that is optimized per each scene, COLMAP provides the best qualitative results, the objects are coherently synthesized, a little blurred. ORB-SLAM (RGB-D) result shows some inconsistencies on the rendering (Fig.~\ref{fig:nerf}-{\em Bottom-right}) and overall less definition than COLMAP, although they both showed a similar trajectory error. Results of FVS and SVS are presented in Fig.~\ref{fig:fvs_nvs}. For both, COLMAP and ORB,  provide less quality than NeRF. It could be explained by the difference in poses configuration w.r.t original methods data on which methods were trained.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.85\linewidth]{images/Nerf.pdf}
  \caption{Qualitative demonstration of the NeRF novel-view synthesis algorithm on new poses, not observed before.}
  \label{fig:nerf}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{images/fvs_svs.pdf}
  \caption{Qualitative demonstration of the FVS and SVS novel-view synthesis algorithms on new poses, not observed before.}
  \label{fig:fvs_nvs}
\end{figure}


==> CVPR'21 Avatar dataset (Camera Ready)/src/07_conclusions.tex <==
\section{Discussion}

One of the questions that this paper raised in the introduction is: {\em Are we ready to calculate handled trajectories in the wild and convert them into 3D portraits of people?}

%Marsel \mf{here should be common answer, only after we can talk about VI}
%Marsel \mf{Or I didn't get the question and word ONLINE should be added explicitly}

Real time VI methods do not perform as accurately as V methods (some of them not real-time). Still, the accuracy achieved is remarkable, providing very accurate trajectories; probably, they could be better if IMUs were properly initialized.

Despite 
%Marsel \mf{which?}
their accuracy, the results obtained on the applications (NeRF and reconstruction) could be improved.
This question is to be explored, but our qualitative results hint that trajectory error is not perfectly correlated with the downstream task, either for synthesis or for reconstruction. An explanation can be the photo-metric consistency, which is more important than the trajectory error.
A corollary of this: perhaps the solution is not to jointly optimize trajectories and maps, but simply optimize the map, allowing for small disturbances on the camera poses from a reasonable initial solution.
We plan to further investigate this issue. % with more trajectories and more methods to compare.

{\bf Potential Negative Societal Impact.}
Realistic human data are required to achieve a future of immersive VR and tele-presence. However, there are other potentially dangerous uses of these technology such as identity theft or fake news.

{\bf Acknowledgments.} This research is based on the work supported by Samsung Research, Samsung Electronics.



==> CVPR'21 Avatar dataset (Camera Ready)/src/archive.tex <==
Novel view synthesis
\cite{mildenhall2019local, yoon2020novel, sevastopolsky2020relightable, Zhou2018Stereo}

Radiance fields
\cite{mildenhall2020nerf, gao2020portrait, liu2020neuralvoxels}

Volumetric representations
\cite{lombardi2019neuralvolumes, niemeyer2020differentiable, sitzmann2019scene, park2019deepsdf}

Nerf + Dynamics, Portraits
\cite{xian2021space, pumarola2021d, park2021nerfies, gafni2021dynamic}

\kp{the one I sent to you}
\cite{gao2020portrait} - novel view and fov synthesis from single image.
Use self-captured dataset made on a light stage (a lot of cameras and light sources) that contains images, meshes, textures (after processing the images); 70 static subjects with diverse characteristics captured from different poses; Use 3D morphable models (3DMM, probably like one in option 1) to obtain parameters of faces. Camera poses are obtained from light stage equipment.

\kp{just gathering the data}

\kp{Option 1*}

\cite{gafni2021dynamic} - novel pose and expression synthesis from monocular video
Use a dataset of self-captured sequences of facial expressions, include talking, smiling, head rotations;
They require expressions and poses (so no colmap) for each image that are acquired via morphable model (A Morphable Model For The Synthesis Of 3D Faces). The latter uses a database of 3D scans of human faces (acquired with lasers) and a model to provide the required data.

\kp{Categories to be assigned}

\kp{Option 1}
Nerf 4D (position + time)
https://arxiv.org/pdf/2011.12950.pdf

Use dataset (from https://dl.acm.org/doi/pdf/10.1145/3386569.3392377) of images (from video) with depth measurements (estimated using the method in the paper the dataset originates from). Contains humans, animals, furniture. Also train and validate on a synthetic dataset created from animated clips that include humans (https://files.is.tue.mpg.de/black/papers/ButlerECCV2012-corrected.pdf)

\kp{Option 2}
Video reenactment for portraits. 
https://dl.acm.org/doi/pdf/10.1145/3197517.3201283

Use videos from public sources only.

\kp{Option 3}
Image animation using a video.
https://proceedings.neurips.cc/paper/2019/file/31c0b36aef265d9221af80872ceb62f9-Paper.pdf

Datasets used VoxCeleb, Tai-Chi-HD (self-gathered), Fashion-Videos, MGif. All datasets consist of sequences of videos, including those extracted from public sources.

\kp{Option 4}
An alternative to 3DMM. The aim is to 3D regress full facial structure from a 2D image
https://arxiv.org/pdf/1703.07834.pdf

Requires images + 3D scans for training. Use 300W-LP dataset that was made by processing images from 300W dataset (paper called: A semi-automatic methodology for facial landmark annotation). Evaluate on AFLW2000-3D, BU-4DFE, Florence datasets (images + 3D scans of human faces with different expression).

\kp{Option 5}
Few-shot Video-to-Video Synthesis
https://arxiv.org/pdf/1910.12713.pdf

Video synthesis from input videos and few images of a new scene. Use the following datasets with videos: YouTube dancing videos, Street-scene videos, Face videos

\kp{Option 6}
Deep 3D Portrait from a Single Image
https://openaccess.thecvf.com/content_CVPR_2020/papers/Xu_Deep_3D_Portrait_From_a_Single_Image_CVPR_2020_paper.pdf

Recovers 3D geometry of human head from a single image for pose manipulation.
Trained on CelebA, 300W-LP, LFW datasets. 

\kp{Option 7}
Fast Bi-Layer Neural Synthesis of One-Shot Realistic Head Avatars
https://arxiv.org/pdf/2008.10174.pdf

Use datasets VoxCeleb2, VoxCeleb2-HQ that were processed with a facial landmarks detector.

\kp{Option 8}

\cite{park2021nerfies} Nerf with deformation field. Collect their own dataset with a synch-ed stereo rig and run colmap to recover poses. Although D-Nerf they still use colmap for poses. Also they mention that dataset of \cite{yoon2020novel} is not representative enough and has exaggerated frame-to-frame motion.

\kp{Option 9}
NSV for dynamic scenes
\cite{yoon2020novel} capture their own dataset. 1) collect short dynamic sequences with samsung gn10, 2) collect videos with static rig of 12 GoPro cameras. Use colmap for obtaining poses.


\section{Recording Platform}
\label{sec:sys}
\ak{Whole section requires to be shorten!!!}

Our dataset aims to provide human portrait data in the realistic environments captured on a middle-range smartphone for 3D reconstruction and rendering applications. To meet those requirements, we have designed a portable handheld platform with a Samsung S10e smartphone and a high-quality depth sensor Azure Kinect DK. A common view of the system is presented in Fig.~\ref{fig:system_common_view}. Main design solutions of recording platform are mentioned in Sec.~\ref{sec:system_design}. Heterogeneity of smartphone and depth camera adds additional challenge on time synchronization during the recording that we solve as described in Sec.~\ref{sec:sys_sync}. Details on extrinsics and intrinsics calibration parameters for our platform are discussed in Sec.~\ref{sec:sys_calib}. 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{images/common_view.jpg}
  \caption{\mf{I'll edit figure a little to avoid 100\% copy paste from bandeja paper}Front and back view of the recording platform}
  \label{fig:system_common_view}
\end{figure}

\mf{I exchanged sync and design solutions to naturally answer question Why these design solutions?}

\subsection{Time \mf{and frame?} synchronization}
\label{sec:sys_sync}

\mf{looks too long sentence to follow, hard for me. If you agree I will divide it in the next iteration}
Specifics of our recording case~--- dynamic camera movements close to real-life handheld capture and scene with dynamic parts (eyes, small movements of the person \mf{maybe add: because of breath, coordination, heart beats})~--- arise additional requirements for sync quality between depth and smartphone camera, because \mf{in case (when) (without these words it may look like it is right our case with out of sync)} frames from both sensors captured at slightly different time could not accurately correspond. Synchronization of capturing frames from smartphone and depth \mf{cameras?} \mf{of our system} is a two-step process. Firstly, time domains between two sensors should be synchronized. We do this via Twist-n-Sync algorithm~\cite{faizullin2021twist} \mf{that is not affected by network asymmetry as network-based protocols like NTP are}\st{, less prone to network asymmetry in comparison to network-based protocols like NTP}. Second step -- synchronize moments of frame capturing from both sensors. For that we start record on the smartphone, obtain its phase parameters via remote API interface and adopt depth triggering to this phase in common time domain.

\subsection{Design solutions}
\label{sec:system_design}

\textbf{Depth} The high-quality external \mf{depth camera}\st{sensor} was chosen instead of the smartphone with a built-in \mf{sensor}\st{depth camera} because \mf{\st{of the following reasons:}} (i) modern smartphone depth images are still not \mf{as} high\mf{-} quality as external depth sensors that limit their usage as a source of ground truth information, and (ii) it is not possible to record RGB and depth tracks \mf{by}\st{from} the smartphone on high frequency simultaneously. \mf{Maybe skip the following sentence:}\mf{An} External depth sensor could also be a support for trajectory estimation methods by running RGBD SLAM. 

\mf{I would completely remove this paragraph content and cite bandeja paper. However, I would add:\\
For launching synchronous data capturing, additional hardware has been/is used: mini PC, MCU(microcontroller unit)-board, standalone IMU. }
\textbf{Hardware} In our system configuration, we use the Samsung S10e smartphone, Azure Kinect DK depth camera (other sensors besides depth are not used), standalone MPU-9150 IMU-sensor, NUC mini PC, powered by Ubuntu 18.04 OS, Intel(R) Core(TM) i7-10710U CPU @ 6-Core 1.1GHz, 16 GB DDR4-2666MHz RAM., 500 GB M.2 SSD storage, STM32F4DISCOVERY MCU platform based on STM32F407 MCU. The smartphone is powered by Android 10 OS and utilizes a standard  camera for video recording with 1920$\times$1080 pixel resolution and a 30 fps frame rate. The smartphone IMU sensor (gyroscope, accelerometer) collects inertial measurements at 500 Hz data rate. The depth camera is set up to capture depth images with narrow field of view with 640$\times$576 pixel resolution and a 5 fps frame rate. 

\textbf{Software} The platform software consists of two main components~--- (i) ROS-based software that \mf{is ran. word runs/is running also fine (programma rabotaet na computere)} \st{is run} on the NUC laptop and (ii) OpenCamera Sensors~\ak{cite}\mf{check this \cite{opencamsensors} or use \footnote{\url{https://github.com/MobileRoboticsSkoltech/OpenCamera-Sensors}}} application that \mf{is ran. runs/is running also fine}\st{is run} on the smartphone. ROS-based software is the main entry point in the data collection process~--- it controls the start and stop of the recording, triggers depth \mf{better frames/images because triggers every frame}capturing via MCU board, interacts with the smartphone over Wi-Fi for synchronization of smartphone camera \st{stream} and depth stream\mf{s}. \mf{Such? Do not see clear relation of the part above with this word. I would use The}Such system configuration allows us to start and stop the recording process via SSH independently from the operator that carries the platform. Data collection on the smartphone is performed via OpenCamera Sensors application, which supports remote control interface via the network, provides synchronization of smartphone camera and IMU sensors, and shares information about camera phase parameters for \mf{\st{adapting depth camera triggers}} synchronous frame capturing with depth.

\subsection{Calibration}
\label{sec:sys_calib}

\ak{Some intro words}

\subsubsection{Smartphone Sensors Calibration}

\ak{Marsel, your turn: about camera, IMU and their relat transform}

\mf{for now we may need to explain, why we do not use kalibr~\cite{rehder2016extending} for smartphone camera intrinsic calibration}

% \ak{From Konstantin, but let's describe last exp}
% In order to find intrinsic parameters and to amend for the distortions of the cameras, we perform a calibration procedure. We use a $8 \times 6$ chessboard calibration pattern with a square size of 55 mm and calibration utilities provided by OpenCV \cite{2015opencv} that are based on the method described in \cite{zhang2000flexible} to determine the required parameters. They are focal length, optical center, and 8 distortion coefficients. We have chosen a rational distortion model with 8 coefficients because of the poor performance of the 5-coefficient model. We explain it by the huge geometric imperfection of smartphone camera lenses.


\subsubsection{Smartphone Camera to Depth Camera Calibration}
\label{sec:calib_cam2depth}
To get relative transformation between depth camera and smartphone camera we employ the following procedure. Firstly, we detect chessboard corners on the calibration pattern with both cameras. Next, we estimate the poses of detected chessboard corners in the local system of coordinates for each camera. For Azure, to translate keypoints from the image plane to the local camera coordinates we use provided depth measurements, whereas for Samsung S10e we solve the PnP problem using IPPE \cite{collins2014infinitesimal} implemented in OpenCV \cite{2015opencv}. Then, we estimate the initial transformation between two point clouds of chessboard corners using the method described in \cite{horn1988closed}. We have found that it gives a slightly more accurate initial guess than \cite{arun1987least} due to the planarity of two sets of points. The obtained initial guess is usually very coarse due to the significant difference in the intrinsic parameters of the cameras. Thus, to ensure that the transformation correctly maps keypoints between images recorded by both cameras we further refine the parameters of the initial transformation subject to epipolar constraints between the keypoints using LM. As epipolar constraints influence only the direction of the relative translation between cameras poses, we additionally perform a line search along the direction to acquire the magnitude. The final transformation is produced by averaging several refined estimates where the recorded calibration pattern is stationed at different distances from the cameras.





\section{Dataset}

Our dataset contains 1000 records of 200 people, captured in different native locations and poses with relightning; the summary duration of all tracks is 11 hours and 6 minutes, and the summary length is 6610 meters. Every record consists of synchronized smartphone data (full HD RGB video, \mf{timestamped} accelerometer and gyroscope measurements, flash timestamps) and depth images from external high-quality depth sensor. The dataset also contains reference ground truth trajectories of the smartphone camera and segmentation masks for the persons. Data parameters and sampling \mf{rates}\st{frequency} are presented in Tab.~\ref{tab:dataset}. This section describes \st{the collection process, statistics on the collected data, and how we obtained person masks and GT trajectories when post-processed the recording data}\mf{the data collection process, collected data statistics, and person masks and ground truth trajectories generation procedures}.

\begin{table}
  \centering
  \begin{tabular}{@{}lcr@{}}
    \toprule
    Type & Data & Properties \\
    \midrule
    Smartphone & RGB video & 1920 $\times$ 1080, 30 Hz \\
    & Gyroscope & \ak{??}, 500 Hz \\
    & Accelerometer & \ak{??}, 500 Hz \\
    & Flash timestamps & \ak{??}, 1 Hz \\ 
    & Frame timestamps & \ak{??}, 30 Hz \\
    % \midrule
    Depth camera & Depth frames & 640 $\times$ 576, 5 Hz \\
    \midrule
    Segmentation masks & RGB video & 1920 $\times$ 1080, 30 Hz \\
    % \midrule
    Ground truth & 6D poses & 5 Hz \\
    \bottomrule
  \end{tabular}
  \caption{Recorded data}
  \label{tab:dataset}
\end{table}

\subsection{Collection process}

\mf{choose single tense if possible}
During \st{the}\mf{a} recording process, the subjects were asked to stand still; the platform operator carried a recording platform around the person at the subject's face height as depicted in Fig.~\ref{fig:recording_process}. The recording trajectory begins in front of the person to capture the whole scene, then operator moves to the right side of the person and makes four full semi-circles of 140-160 degrees angles around the person. Resulted recording trajectory is schematically demonstrated \st{on the}\mf{always only in} Fig.~\ak{add}. The borders of every semi-circle are marked by the external operator that sends a special signal to the recording platform through SSH during the data collection. In post-processing \mf{stage?}, the whole trajectory could be split into separate sub-trajectories.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/Recording.pdf}
%   \caption{Show recording process}
%   \label{fig:recording_process}
% \end{figure}

Every person was captured in 5 different poses~--- 3 in a standing position (straight, hand on hips, with head turned) and 2 in a sitting position (straight, with head turned), as depicted in Fig.~\ref{fig:recording_poses}. \st{Standing positions were captured from a distance of 2 meters, sitting positions from a distance of 1 meter.}
\mf{Standing and sitting positions were captured from a distance of about 2 and 1 m respectively.} 
During the recording, blinking flash on the smartphone was turned on with a frequency of 1 Hz to relight avatar surfaces. Effect of relightning is more distinguishable on sitting positions since they were captured from less distance.

Data collection was performed in 5 different locations in native indoor\st{s}\mf{adjective, not adverb} environments: cafeteria, lab, office, campus entrance, and student council. Their common view is demonstrated in Fig.~\ref{fig:diversity}.

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/Poses.pdf}
%   \caption{Show poses}
%   \label{fig:recording_poses}
% \end{figure*}

\subsection{Statistics}

Our dataset contains 200 people of different gender and appearance, captured in 5 different locations, every person was captured in 5 different poses. Fig.~\ref{fig:dataset_stat} presents information on distribution on gender. Statistics over locations are demonstrated in Fig.~\ref{fig:dataset_stat}. Since 3D reconstruction and rendering of humans is complicated on the parts with glasses and hairs (beard, voluminous hairstyles), we also added labels for this; their statistics are presented in Fig.~\ref{fig:dataset_stat}. 

The average length of the trajectories for staying position is 7.14 meters, for sitting~--- 5.8 meters. \ak{where to put this?}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/DataStat2.pdf}
%   \caption{Show data stat}
%   \label{fig:dataset_stat}
% \end{figure}

\subsection{Segmentation Masks}

Along with recorded data, we also provide segmentation masks of humans on the images. This information could be used for filtering out potentially dynamic landmarks of the scene on the trajectory estimation step (blinking eyes, subject movements) as demonstrated in \ak{link to eval?} or for separation of avatar parts from the scene for only-person 3D reconstruction.

For this task, we designed a semi-automated labeling process, based on U2-Net~\cite{qin2020u2} that was pre-trained on people masks from Supervisely Person Dataset~\ak{cite}. Usage of this method on our data overestimates the person mask, also covering some parts of the background as depicted in Fig.~\ref{fig:dataset_masks}. To filter them out, we use corresponding depth information and DBSCAN clustering of masked part of the depth component, discarding scene parts not related to the foreground. Finally, segmentation results were assessed visually by labelers.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/mask_pipeline.pdf}
%   \caption{Show mask pipelines}
%   \label{fig:dataset_masks}
% \end{figure}

\subsection{Ground Truth Trajectories}
\label{sec:gt}

\kp{TODO. Motivation on the choice of the method for ground-truth generation. Proposals for sections: 4.4, 4.4.1, 4.4.2 START}

The majority of the sequences of the proposed dataset (see Fig. \ref{fig:dataset_stat}) were captured in public places or areas where either applying conventional methods of acquiring ground truth poses is not feasible or a method disrupts the nativity of the surroundings (e.g. visual markers). Hence following \cite{} we provide pseudo-ground truth poses (referred to as ground truth next in the text) that are calculated based on the collected sensors data.

In order to make the best use of the gathered data for the purpose of the ground truth calculation, we considered SLAM algorithms that work with RGB-D \kp{if we have evaluation of orb-slam3 with inertial sensors then add IMU here as well}. Based on the evaluation of RGB-D SLAM methods done in \cite{zhang2021survey} we chose ORB-SLAM2 \cite{} as it has the lowest ATE. \kp{why it is important? because nerfs and other our applications (which?) like good poses; need to elaborate with references}. In our implementation, we use RGB modification of ORB-SLAM3 \cite{campos2021orb} that works in the same way as ORB-SLAM2 \kp{right?}. We provide RGB frames and depth information to the algorithm from the smartphone and from the external depth camera respectively. Depth frames are transformed to the RGB frames reference system of coordinates using the calibration (see section \ref{sec:calib_cam2depth}).
\kp{A few words about BundleFusion?}

In the area of 3D rendering that the proposed dataset is aimed at, a Structure-from-Motion (SfM) pipeline COLMAP \cite{schoenberger2016sfm, schoenberger2016mvs} is usually employed to get ground truth poses \kp{nerf staff, 3D rendering; find an appropriate term, verify usage of COLMAP}. Likewise, COLMAP is also used as a ground truth acquisition method for VIO benchmarks \cite{} \kp{+1-2 more citations}. To our knowledge, there is no thorough study that compares pose estimation accuracy of existing SLAM and SfM methods \kp{is there?}, thus, to \kp{what for? motivation should be based on the examples above} we in addition to ORB-SLAM2 poses provide ground truth poses obtained from COLMAP 3D reconstructions. A COLMAP reconstruction is defined up to a scale factor so in order to get the metric scale for ground truth poses we \kp{Here describe alignment method and recovery of the scaling factor}

\kp{How do we treat each of the ground truth tracks (orb, colmap)? What is their intention? Which one to prioritize and why? Elaborate} 

To assess the accuracy of the ground truth poses we similar to \cite{} record several testing sequences in the laboratory environment where the use of a more accurate ground truth acquisition method is possible. In particular, we utilize OptiTrack MoCap system to record \kp{how much seqs do we have?} testing sequences. \kp{Adapt stuff from 4.4.2 here}

\kp{conclusions and error estimates based on the previous paragraph}

\kp{END}

Additionally, we deliver reference ground truth trajectories that were obtained with ORB-SLAM 3~\cite{campos2021orb} (RGBD modification) method~---State of The Art RGBD method on a wide variety of benchmark datasets~\cite{zhang2021survey}. In our variant, it uses RGB information from the smartphone and depth information from the external depth camera, re-projected onto smartphone coordinate frame, using calibrated intrinsics and extrinsics from Sec.~\ak{add}. In this section, we explain the motivation for using ORB SLAM and provide quantitative results on the quality of trajectories.

\subsubsection{Motivation on ORB-SLAM}

The de-facto standard tool for calculating camera poses for further usage in dense 3D reconstruction or rendering tasks is extrinsic parameters from sparse reconstruction step of COLMAP~\cite{schoenberger2016sfm, schoenberger2016mvs}. It is based on Bundle Adjustment and SIFT features; both of these components introduce significant computational complexity and border close to real-time performance. Additionally, COLMAP doesn't provide proper scaling to real-world coordinates \ak{why, explain}. Considering those properties and the high accuracy of RGBD modification of ORB SLAM on a wide variety of data, we considered it the main contender for COLMAP.

\subsubsection{Full-reference evaluation}

To compare quality of trajectories from ORB SLAM 3 and COLMAP, we recorded 5 records of one person in common dataset format using OptiTrack motion capture system~(mocap) as ground truth that provides sub-millimeter accuracy. Mocap was synchronized with the platform in offline by Twist-n-Sync algorithm~\cite{faizullin2021twist}. Since the algorithm is based on angular velocities analysis, the mocap velocity was extracted by finite difference of measured angle. ~\ak{MARSEL, name, accuracy, way to sync}\mf{DONE}. To calculate error statistics, we used implementation of Absolute Pose Error (APE) and Relative Pose Error (RPE) metrics from evo tool~\cite{grupp2017evo}. Before calculating APE, trajectories were aligned by Umeyama alignment. COLMAP trajectories were additionally scaled during Umeyama alignment. Because landmarks on person body are potentially dynamic (person can breath, blink), we considered three modifications of ORB SLAM -- not using person mask, using mask for background, using mask for person. Tab.~\ref{fig:eval_mocap} presents results of evaluation those ORB SLAM variants and COLMAP.

\ak{Explain why we don't provide APE-rot}

\ak{Results: ORB outperforms COLMAP on RPE for both rotation and translation. COLMAP with scaling outperforms ORB on APE because scaling overfits error, ORB with scaling gives comparable results (here maps from pcs could be demonstrated). Masks doesn't help, but on background they are comparable to original one. }

\begin{table}
  \centering
  \begin{tabular}{@{}lccr@{}}
    \toprule
    Method & APE-transl & RPE-rot & RPE-transl \\
    \midrule
    & Record 1 & & \\
    \midrule
    ORB & 0.0155 &	3.8390 & 0.0252 \\
    ORB (person) & 0.0192 &	3.8629	 & 0.0286 \\
    ORB (background) & 0.0290 &	3.8450 & 0.0263 \\
    COLMAP (with scaling) & 0.0073 &	3.8466	 & 0.0251 \\
    ORB (with scaling) & 0.0071 &	3.8390 & 0.0249 \\
    ORB + ICP & 0.0102 &	3.8274 & 0.0248 \\
    \midrule
    & Record 2 & & \\
    \midrule
    ORB &	0.0108 &	3.9622 &	0.0247 \\
    ORB (person) &	0.0182 &	3.9753 &	0.0262 \\
    ORB (background) &	0.0199 &	3.9767 &	0.0255 \\
    COLMAP (with scaling) &	0.0077 &	3.9751 &	0.0246 \\
    ORB (with scaling) &	0.0075 &	3.9622 &	0.0245 \\
    ORB + ICP ref &	0.0065 &	3.9559 &	0.0244 \\
    \midrule
    & Record 3 & & \\
    \midrule
    ORB &	0.0089 &	4.2945 &	0.0250 \\
    ORB (person) &	0.0150 &	4.3125 &	0.0275 \\
    ORB (background) &	0.0226 &	4.3302 &	0.0271 \\
    COLMAP (with scaling) &	0.0091 &	4.2977 &	0.0252 \\
    ORB (with scaling) &	0.0086 &	4.2945 &	0.0249 \\
    ORB + ICP ref &	0.0106 &	4.2996 &	0.0248 \\
        \midrule
    & Record 4 & & \\
    \midrule
    ORB &	0.0115 &	5.0057 &	0.0405 \\
    ORB (person) & - &	- &	- \\
    ORB (background) &	0.0247 &	5.0268 &	0.0409 \\
    COLMAP (with scaling) &	0.0070 &	5.0183 &	0.0403 \\
    ORB (with scaling) &	0.0067 &	5.0057 &	0.0400 \\
    ORB + ICP ref &	0.0055 &	5.0028 &	0.0402 \\
        \midrule
    & Record 5 & & \\
    \midrule
    ORB &	0.0095 &	4.9295 &	0.0368 \\
    ORB (person) &	0.3196 &	5.4726 &	0.0823 \\
    ORB (background) &	0.0180 &	4.9435 &	0.0371 \\
    COLMAP (with scaling) &	0.0053 &	4.9371 &	0.0367 \\
    ORB (with scaling) &	0.0053 &	4.9295 &	0.0364 \\
    ORB + ICP ref &	0.0056 &	4.9336 &	0.0368 \\
    \bottomrule
  \end{tabular}
  \caption{Eval}
  \label{tab:eval_mocap}
\end{table}

\subsubsection{Scaling trajectories}



==> CVPR'21 Avatar dataset (Camera Ready)/src/trash.tex <==

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lccr@{}}
%     \toprule
%     Method & APE-transl & RPE-rot & RPE-transl \\
%     \midrule
%     & Record 1 & & \\
%     \midrule
%     ORB & 0.0155 &	3.8390 & 0.0252 \\
%     ORB (person) & 0.0192 &	3.8629	 & 0.0286 \\
%     ORB (background) & 0.0290 &	3.8450 & 0.0263 \\
%     COLMAP (with scaling) & 0.0073 &	3.8466	 & 0.0251 \\
%     ORB (with scaling) & 0.0071 &	3.8390 & 0.0249 \\
%     ORB + ICP & 0.0102 &	3.8274 & 0.0248 \\
%     \midrule
%     & Record 2 & & \\
%     \midrule
%     ORB &	0.0108 &	3.9622 &	0.0247 \\
%     ORB (person) &	0.0182 &	3.9753 &	0.0262 \\
%     ORB (background) &	0.0199 &	3.9767 &	0.0255 \\
%     COLMAP (with scaling) &	0.0077 &	3.9751 &	0.0246 \\
%     ORB (with scaling) &	0.0075 &	3.9622 &	0.0245 \\
%     ORB + ICP ref &	0.0065 &	3.9559 &	0.0244 \\
%     \midrule
%     & Record 3 & & \\
%     \midrule
%     ORB &	0.0089 &	4.2945 &	0.0250 \\
%     ORB (person) &	0.0150 &	4.3125 &	0.0275 \\
%     ORB (background) &	0.0226 &	4.3302 &	0.0271 \\
%     COLMAP (with scaling) &	0.0091 &	4.2977 &	0.0252 \\
%     ORB (with scaling) &	0.0086 &	4.2945 &	0.0249 \\
%     ORB + ICP ref &	0.0106 &	4.2996 &	0.0248 \\
%         \midrule
%     & Record 4 & & \\
%     \midrule
%     ORB &	0.0115 &	5.0057 &	0.0405 \\
%     ORB (person) & - &	- &	- \\
%     ORB (background) &	0.0247 &	5.0268 &	0.0409 \\
%     COLMAP (with scaling) &	0.0070 &	5.0183 &	0.0403 \\
%     ORB (with scaling) &	0.0067 &	5.0057 &	0.0400 \\
%     ORB + ICP ref &	0.0055 &	5.0028 &	0.0402 \\
%         \midrule
%     & Record 5 & & \\
%     \midrule
%     ORB &	0.0095 &	4.9295 &	0.0368 \\
%     ORB (person) &	0.3196 &	5.4726 &	0.0823 \\
%     ORB (background) &	0.0180 &	4.9435 &	0.0371 \\
%     COLMAP (with scaling) &	0.0053 &	4.9371 &	0.0367 \\
%     ORB (with scaling) &	0.0053 &	4.9295 &	0.0364 \\
%     ORB + ICP ref &	0.0056 &	4.9336 &	0.0368 \\
%     \bottomrule
%   \end{tabular}
%   \caption{Eval}
%   \label{tab:eval_mocap}
% \end{table}


% \subsubsection{Motivation on ORB-SLAM}

% The de-facto standard tool for calculating camera poses for further usage in dense 3D reconstruction or rendering tasks is extrinsic parameters from sparse reconstruction step of COLMAP~\cite{schoenberger2016sfm, schoenberger2016mvs}. It is based on Bundle Adjustment and SIFT features; both of these components introduce significant computational complexity and border close to real-time performance. Additionally, COLMAP doesn't provide proper scaling to real-world coordinates \ak{why, explain}. Considering those properties and the high accuracy of RGBD modification of ORB SLAM on a wide variety of data, we considered it the main contender for COLMAP.

% \subsubsection{Full-reference evaluation}

% To compare quality of trajectories from ORB SLAM 3 and COLMAP, we recorded 5 records of one person in common dataset format using OptiTrack motion capture system~(mocap) as ground truth that provides sub-millimeter accuracy. Mocap was synchronized with the platform in offline by Twist-n-Sync algorithm~\cite{faizullin2021twist}. Since the algorithm is based on angular velocities analysis, the mocap velocity was extracted by finite difference of measured angle. ~\ak{MARSEL, name, accuracy, way to sync}\mf{DONE}. To calculate error statistics, we used implementation of Absolute Pose Error (APE) and Relative Pose Error (RPE) metrics from evo tool~\cite{grupp2017evo}. Before calculating APE, trajectories were aligned by Umeyama alignment. COLMAP trajectories were additionally scaled during Umeyama alignment. Because landmarks on person body are potentially dynamic (person can breath, blink), we considered three modifications of ORB SLAM -- not using person mask, using mask for background, using mask for person. Tab.~\ref{fig:eval_mocap} presents results of evaluation those ORB SLAM variants and COLMAP.

% \ak{Explain why we don't provide APE-rot}

% \ak{Results: ORB outperforms COLMAP on RPE for both rotation and translation. COLMAP with scaling outperforms ORB on APE because scaling overfits error, ORB with scaling gives comparable results (here maps from pcs could be demonstrated). Masks doesn't help, but on background they are comparable to original one. }

% \subsubsection{Scaling trajectories}

\ak{Motivation on SfM and RGBD}
\textbf{RGBD}  \kp{why it is important? because nerfs and other our applications (which?) like good poses; need to elaborate with references}. In our implementation, we use RGB modification of ORB-SLAM3 \cite{campos2021orb} that works in the same way as ORB-SLAM2 \kp{right?}. We provide RGB frames and depth information to the algorithm from the smartphone and from the external depth camera respectively. Depth frames are transformed to the RGB frames reference system of coordinates using the calibration (see section \ref{sec:calib_cam2depth}).
\kp{A few words about BundleFusion?}

\textbf{SfM} In the area of 3D reconstruction that the proposed dataset is aimed at, a Structure-from-Motion (SfM) pipeline COLMAP \cite{schoenberger2016sfm, schoenberger2016mvs} is usually employed to get ground truth poses \kp{nerf staff, 3D rendering; find an appropriate term, verify usage of COLMAP}. Likewise, COLMAP is also used as a ground truth acquisition method for VIO benchmarks \cite{} \kp{+1-2 more citations}. To our knowledge, there is no thorough study that compares pose estimation accuracy of existing SLAM and SfM. A COLMAP reconstruction  so in order to get the metric scale for ground truth poses we \kp{Here describe alignment method and recovery of the scaling factor}

% \kp{How do we treat each of the ground truth tracks (orb, colmap)? What is their intention? Which one to prioritize and why? Elaborate} 

%  \kp{Adapt stuff from 4.4.2 here}

% \kp{conclusions and error estimates based on the previous paragraph}

% Additionally, we deliver reference ground truth trajectories that were obtained with ORB-SLAM 3~\cite{campos2021orb} (RGBD modification) method~---State of The Art RGBD method on a wide variety of benchmark datasets~\cite{zhang2021survey}. In our variant, it uses RGB information from the smartphone and depth information from the external depth camera, re-projected onto smartphone coordinate frame, using calibrated intrinsics and extrinsics from Sec.~\ak{add}. In this section, we explain the motivation for using ORB SLAM and provide quantitative results on the quality of trajectories.


%\begin{table}
%  \fontsize{9.5}{9}\selectfont
%  \centering
%  \begin{tabular}{@{}lcr@{}}
%    \toprule
%    Type & Data & Properties \\
%    \midrule
%    Smartphone & RGB video & 1920 $\times$ 1080, 30 Hz \\
%    & Gyroscope & , 500 Hz \\
%    & Accelerometer & , 500 Hz \\
%    & Flash timestamps & \ak{??}, 1 Hz \\ 
%    % \midrule
%    Depth camera & Depth frames & 640 $\times$ 576, 5 Hz \\
%    \midrule
%    Segment. masks & RGB video & 1920 $\times$ 1080, 30 Hz \\
%    % \midrule
%    Ground truth & 3D poses & 5 Hz \\
%    \bottomrule
%  \end{tabular}
%  \caption{Recorded data \gf{what is new wrt the table at RW?}}
%  \label{tab:dataset}
%\end{table}

==> src/archive.tex <==
Novel view synthesis
\cite{mildenhall2019local, yoon2020novel, sevastopolsky2020relightable, Zhou2018Stereo}

Radiance fields
\cite{mildenhall2020nerf, gao2020portrait, liu2020neuralvoxels}

Volumetric representations
\cite{lombardi2019neuralvolumes, niemeyer2020differentiable, sitzmann2019scene, park2019deepsdf}

Nerf + Dynamics, Portraits
\cite{xian2021space, pumarola2021d, park2021nerfies, gafni2021dynamic}

\kp{the one I sent to you}
\cite{gao2020portrait} - novel view and fov synthesis from single image.
Use self-captured dataset made on a light stage (a lot of cameras and light sources) that contains images, meshes, textures (after processing the images); 70 static subjects with diverse characteristics captured from different poses; Use 3D morphable models (3DMM, probably like one in option 1) to obtain parameters of faces. Camera poses are obtained from light stage equipment.

\kp{just gathering the data}

\kp{Option 1*}

\cite{gafni2021dynamic} - novel pose and expression synthesis from monocular video
Use a dataset of self-captured sequences of facial expressions, include talking, smiling, head rotations;
They require expressions and poses (so no colmap) for each image that are acquired via morphable model (A Morphable Model For The Synthesis Of 3D Faces). The latter uses a database of 3D scans of human faces (acquired with lasers) and a model to provide the required data.

\kp{Categories to be assigned}

\kp{Option 1}
Nerf 4D (position + time)
https://arxiv.org/pdf/2011.12950.pdf

Use dataset (from https://dl.acm.org/doi/pdf/10.1145/3386569.3392377) of images (from video) with depth measurements (estimated using the method in the paper the dataset originates from). Contains humans, animals, furniture. Also train and validate on a synthetic dataset created from animated clips that include humans (https://files.is.tue.mpg.de/black/papers/ButlerECCV2012-corrected.pdf)

\kp{Option 2}
Video reenactment for portraits. 
https://dl.acm.org/doi/pdf/10.1145/3197517.3201283

Use videos from public sources only.

\kp{Option 3}
Image animation using a video.
https://proceedings.neurips.cc/paper/2019/file/31c0b36aef265d9221af80872ceb62f9-Paper.pdf

Datasets used VoxCeleb, Tai-Chi-HD (self-gathered), Fashion-Videos, MGif. All datasets consist of sequences of videos, including those extracted from public sources.

\kp{Option 4}
An alternative to 3DMM. The aim is to 3D regress full facial structure from a 2D image
https://arxiv.org/pdf/1703.07834.pdf

Requires images + 3D scans for training. Use 300W-LP dataset that was made by processing images from 300W dataset (paper called: A semi-automatic methodology for facial landmark annotation). Evaluate on AFLW2000-3D, BU-4DFE, Florence datasets (images + 3D scans of human faces with different expression).

\kp{Option 5}
Few-shot Video-to-Video Synthesis
https://arxiv.org/pdf/1910.12713.pdf

Video synthesis from input videos and few images of a new scene. Use the following datasets with videos: YouTube dancing videos, Street-scene videos, Face videos

\kp{Option 6}
Deep 3D Portrait from a Single Image
https://openaccess.thecvf.com/content_CVPR_2020/papers/Xu_Deep_3D_Portrait_From_a_Single_Image_CVPR_2020_paper.pdf

Recovers 3D geometry of human head from a single image for pose manipulation.
Trained on CelebA, 300W-LP, LFW datasets. 

\kp{Option 7}
Fast Bi-Layer Neural Synthesis of One-Shot Realistic Head Avatars
https://arxiv.org/pdf/2008.10174.pdf

Use datasets VoxCeleb2, VoxCeleb2-HQ that were processed with a facial landmarks detector.

\kp{Option 8}

\cite{park2021nerfies} Nerf with deformation field. Collect their own dataset with a synch-ed stereo rig and run colmap to recover poses. Although D-Nerf they still use colmap for poses. Also they mention that dataset of \cite{yoon2020novel} is not representative enough and has exaggerated frame-to-frame motion.

\kp{Option 9}
NSV for dynamic scenes
\cite{yoon2020novel} capture their own dataset. 1) collect short dynamic sequences with samsung gn10, 2) collect videos with static rig of 12 GoPro cameras. Use colmap for obtaining poses.


\section{Recording Platform}
\label{sec:sys}
\ak{Whole section requires to be shorten!!!}

Our dataset aims to provide human portrait data in the realistic environments captured on a middle-range smartphone for 3D reconstruction and rendering applications. To meet those requirements, we have designed a portable handheld platform with a Samsung S10e smartphone and a high-quality depth sensor Azure Kinect DK. A common view of the system is presented in Fig.~\ref{fig:system_common_view}. Main design solutions of recording platform are mentioned in Sec.~\ref{sec:system_design}. Heterogeneity of smartphone and depth camera adds additional challenge on time synchronization during the recording that we solve as described in Sec.~\ref{sec:sys_sync}. Details on extrinsics and intrinsics calibration parameters for our platform are discussed in Sec.~\ref{sec:sys_calib}. 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{images/common_view.jpg}
  \caption{\mf{I'll edit figure a little to avoid 100\% copy paste from bandeja paper}Front and back view of the recording platform}
  \label{fig:system_common_view}
\end{figure}

\mf{I exchanged sync and design solutions to naturally answer question Why these design solutions?}

\subsection{Time \mf{and frame?} synchronization}
\label{sec:sys_sync}

\mf{looks too long sentence to follow, hard for me. If you agree I will divide it in the next iteration}
Specifics of our recording case~--- dynamic camera movements close to real-life handheld capture and scene with dynamic parts (eyes, small movements of the person \mf{maybe add: because of breath, coordination, heart beats})~--- arise additional requirements for sync quality between depth and smartphone camera, because \mf{in case (when) (without these words it may look like it is right our case with out of sync)} frames from both sensors captured at slightly different time could not accurately correspond. Synchronization of capturing frames from smartphone and depth \mf{cameras?} \mf{of our system} is a two-step process. Firstly, time domains between two sensors should be synchronized. We do this via Twist-n-Sync algorithm~\cite{faizullin2021twist} \mf{that is not affected by network asymmetry as network-based protocols like NTP are}\st{, less prone to network asymmetry in comparison to network-based protocols like NTP}. Second step -- synchronize moments of frame capturing from both sensors. For that we start record on the smartphone, obtain its phase parameters via remote API interface and adopt depth triggering to this phase in common time domain.

\subsection{Design solutions}
\label{sec:system_design}

\textbf{Depth} The high-quality external \mf{depth camera}\st{sensor} was chosen instead of the smartphone with a built-in \mf{sensor}\st{depth camera} because \mf{\st{of the following reasons:}} (i) modern smartphone depth images are still not \mf{as} high\mf{-} quality as external depth sensors that limit their usage as a source of ground truth information, and (ii) it is not possible to record RGB and depth tracks \mf{by}\st{from} the smartphone on high frequency simultaneously. \mf{Maybe skip the following sentence:}\mf{An} External depth sensor could also be a support for trajectory estimation methods by running RGBD SLAM. 

\mf{I would completely remove this paragraph content and cite bandeja paper. However, I would add:\\
For launching synchronous data capturing, additional hardware has been/is used: mini PC, MCU(microcontroller unit)-board, standalone IMU. }
\textbf{Hardware} In our system configuration, we use the Samsung S10e smartphone, Azure Kinect DK depth camera (other sensors besides depth are not used), standalone MPU-9150 IMU-sensor, NUC mini PC, powered by Ubuntu 18.04 OS, Intel(R) Core(TM) i7-10710U CPU @ 6-Core 1.1GHz, 16 GB DDR4-2666MHz RAM., 500 GB M.2 SSD storage, STM32F4DISCOVERY MCU platform based on STM32F407 MCU. The smartphone is powered by Android 10 OS and utilizes a standard  camera for video recording with 1920$\times$1080 pixel resolution and a 30 fps frame rate. The smartphone IMU sensor (gyroscope, accelerometer) collects inertial measurements at 500 Hz data rate. The depth camera is set up to capture depth images with narrow field of view with 640$\times$576 pixel resolution and a 5 fps frame rate. 

\textbf{Software} The platform software consists of two main components~--- (i) ROS-based software that \mf{is ran. word runs/is running also fine (programma rabotaet na computere)} \st{is run} on the NUC laptop and (ii) OpenCamera Sensors~\ak{cite}\mf{check this \cite{opencamsensors} or use \footnote{\url{https://github.com/MobileRoboticsSkoltech/OpenCamera-Sensors}}} application that \mf{is ran. runs/is running also fine}\st{is run} on the smartphone. ROS-based software is the main entry point in the data collection process~--- it controls the start and stop of the recording, triggers depth \mf{better frames/images because triggers every frame}capturing via MCU board, interacts with the smartphone over Wi-Fi for synchronization of smartphone camera \st{stream} and depth stream\mf{s}. \mf{Such? Do not see clear relation of the part above with this word. I would use The}Such system configuration allows us to start and stop the recording process via SSH independently from the operator that carries the platform. Data collection on the smartphone is performed via OpenCamera Sensors application, which supports remote control interface via the network, provides synchronization of smartphone camera and IMU sensors, and shares information about camera phase parameters for \mf{\st{adapting depth camera triggers}} synchronous frame capturing with depth.

\subsection{Calibration}
\label{sec:sys_calib}

\ak{Some intro words}

\subsubsection{Smartphone Sensors Calibration}

\ak{Marsel, your turn: about camera, IMU and their relat transform}

\mf{for now we may need to explain, why we do not use kalibr~\cite{rehder2016extending} for smartphone camera intrinsic calibration}

% \ak{From Konstantin, but let's describe last exp}
% In order to find intrinsic parameters and to amend for the distortions of the cameras, we perform a calibration procedure. We use a $8 \times 6$ chessboard calibration pattern with a square size of 55 mm and calibration utilities provided by OpenCV \cite{2015opencv} that are based on the method described in \cite{zhang2000flexible} to determine the required parameters. They are focal length, optical center, and 8 distortion coefficients. We have chosen a rational distortion model with 8 coefficients because of the poor performance of the 5-coefficient model. We explain it by the huge geometric imperfection of smartphone camera lenses.


\subsubsection{Smartphone Camera to Depth Camera Calibration}
\label{sec:calib_cam2depth}
To get relative transformation between depth camera and smartphone camera we employ the following procedure. Firstly, we detect chessboard corners on the calibration pattern with both cameras. Next, we estimate the poses of detected chessboard corners in the local system of coordinates for each camera. For Azure, to translate keypoints from the image plane to the local camera coordinates we use provided depth measurements, whereas for Samsung S10e we solve the PnP problem using IPPE \cite{collins2014infinitesimal} implemented in OpenCV \cite{2015opencv}. Then, we estimate the initial transformation between two point clouds of chessboard corners using the method described in \cite{horn1988closed}. We have found that it gives a slightly more accurate initial guess than \cite{arun1987least} due to the planarity of two sets of points. The obtained initial guess is usually very coarse due to the significant difference in the intrinsic parameters of the cameras. Thus, to ensure that the transformation correctly maps keypoints between images recorded by both cameras we further refine the parameters of the initial transformation subject to epipolar constraints between the keypoints using LM. As epipolar constraints influence only the direction of the relative translation between cameras poses, we additionally perform a line search along the direction to acquire the magnitude. The final transformation is produced by averaging several refined estimates where the recorded calibration pattern is stationed at different distances from the cameras.





\section{Dataset}

Our dataset contains 1000 records of 200 people, captured in different native locations and poses with relightning; the summary duration of all tracks is 11 hours and 6 minutes, and the summary length is 6610 meters. Every record consists of synchronized smartphone data (full HD RGB video, \mf{timestamped} accelerometer and gyroscope measurements, flash timestamps) and depth images from external high-quality depth sensor. The dataset also contains reference ground truth trajectories of the smartphone camera and segmentation masks for the persons. Data parameters and sampling \mf{rates}\st{frequency} are presented in Tab.~\ref{tab:dataset}. This section describes \st{the collection process, statistics on the collected data, and how we obtained person masks and GT trajectories when post-processed the recording data}\mf{the data collection process, collected data statistics, and person masks and ground truth trajectories generation procedures}.

\begin{table}
  \centering
  \begin{tabular}{@{}lcr@{}}
    \toprule
    Type & Data & Properties \\
    \midrule
    Smartphone & RGB video & 1920 $\times$ 1080, 30 Hz \\
    & Gyroscope & \ak{??}, 500 Hz \\
    & Accelerometer & \ak{??}, 500 Hz \\
    & Flash timestamps & \ak{??}, 1 Hz \\ 
    & Frame timestamps & \ak{??}, 30 Hz \\
    % \midrule
    Depth camera & Depth frames & 640 $\times$ 576, 5 Hz \\
    \midrule
    Segmentation masks & RGB video & 1920 $\times$ 1080, 30 Hz \\
    % \midrule
    Ground truth & 6D poses & 5 Hz \\
    \bottomrule
  \end{tabular}
  \caption{Recorded data}
  \label{tab:dataset}
\end{table}

\subsection{Collection process}

\mf{choose single tense if possible}
During \st{the}\mf{a} recording process, the subjects were asked to stand still; the platform operator carried a recording platform around the person at the subject's face height as depicted in Fig.~\ref{fig:recording_process}. The recording trajectory begins in front of the person to capture the whole scene, then operator moves to the right side of the person and makes four full semi-circles of 140-160 degrees angles around the person. Resulted recording trajectory is schematically demonstrated \st{on the}\mf{always only in} Fig.~\ak{add}. The borders of every semi-circle are marked by the external operator that sends a special signal to the recording platform through SSH during the data collection. In post-processing \mf{stage?}, the whole trajectory could be split into separate sub-trajectories.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/Recording.pdf}
%   \caption{Show recording process}
%   \label{fig:recording_process}
% \end{figure}

Every person was captured in 5 different poses~--- 3 in a standing position (straight, hand on hips, with head turned) and 2 in a sitting position (straight, with head turned), as depicted in Fig.~\ref{fig:recording_poses}. \st{Standing positions were captured from a distance of 2 meters, sitting positions from a distance of 1 meter.}
\mf{Standing and sitting positions were captured from a distance of about 2 and 1 m respectively.} 
During the recording, blinking flash on the smartphone was turned on with a frequency of 1 Hz to relight avatar surfaces. Effect of relightning is more distinguishable on sitting positions since they were captured from less distance.

Data collection was performed in 5 different locations in native indoor\st{s}\mf{adjective, not adverb} environments: cafeteria, lab, office, campus entrance, and student council. Their common view is demonstrated in Fig.~\ref{fig:diversity}.

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/Poses.pdf}
%   \caption{Show poses}
%   \label{fig:recording_poses}
% \end{figure*}

\subsection{Statistics}

Our dataset contains 200 people of different gender and appearance, captured in 5 different locations, every person was captured in 5 different poses. Fig.~\ref{fig:dataset_stat} presents information on distribution on gender. Statistics over locations are demonstrated in Fig.~\ref{fig:dataset_stat}. Since 3D reconstruction and rendering of humans is complicated on the parts with glasses and hairs (beard, voluminous hairstyles), we also added labels for this; their statistics are presented in Fig.~\ref{fig:dataset_stat}. 

The average length of the trajectories for staying position is 7.14 meters, for sitting~--- 5.8 meters. \ak{where to put this?}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/DataStat2.pdf}
%   \caption{Show data stat}
%   \label{fig:dataset_stat}
% \end{figure}

\subsection{Segmentation Masks}

Along with recorded data, we also provide segmentation masks of humans on the images. This information could be used for filtering out potentially dynamic landmarks of the scene on the trajectory estimation step (blinking eyes, subject movements) as demonstrated in \ak{link to eval?} or for separation of avatar parts from the scene for only-person 3D reconstruction.

For this task, we designed a semi-automated labeling process, based on U2-Net~\cite{qin2020u2} that was pre-trained on people masks from Supervisely Person Dataset~\ak{cite}. Usage of this method on our data overestimates the person mask, also covering some parts of the background as depicted in Fig.~\ref{fig:dataset_masks}. To filter them out, we use corresponding depth information and DBSCAN clustering of masked part of the depth component, discarding scene parts not related to the foreground. Finally, segmentation results were assessed visually by labelers.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.99\linewidth]{images/mask_pipeline.pdf}
%   \caption{Show mask pipelines}
%   \label{fig:dataset_masks}
% \end{figure}

\subsection{Ground Truth Trajectories}
\label{sec:gt}

\kp{TODO. Motivation on the choice of the method for ground-truth generation. Proposals for sections: 4.4, 4.4.1, 4.4.2 START}

The majority of the sequences of the proposed dataset (see Fig. \ref{fig:dataset_stat}) were captured in public places or areas where either applying conventional methods of acquiring ground truth poses is not feasible or a method disrupts the nativity of the surroundings (e.g. visual markers). Hence following \cite{} we provide pseudo-ground truth poses (referred to as ground truth next in the text) that are calculated based on the collected sensors data.

In order to make the best use of the gathered data for the purpose of the ground truth calculation, we considered SLAM algorithms that work with RGB-D \kp{if we have evaluation of orb-slam3 with inertial sensors then add IMU here as well}. Based on the evaluation of RGB-D SLAM methods done in \cite{zhang2021survey} we chose ORB-SLAM2 \cite{} as it has the lowest ATE. \kp{why it is important? because nerfs and other our applications (which?) like good poses; need to elaborate with references}. In our implementation, we use RGB modification of ORB-SLAM3 \cite{campos2021orb} that works in the same way as ORB-SLAM2 \kp{right?}. We provide RGB frames and depth information to the algorithm from the smartphone and from the external depth camera respectively. Depth frames are transformed to the RGB frames reference system of coordinates using the calibration (see section \ref{sec:calib_cam2depth}).
\kp{A few words about BundleFusion?}

In the area of 3D rendering that the proposed dataset is aimed at, a Structure-from-Motion (SfM) pipeline COLMAP \cite{schoenberger2016sfm, schoenberger2016mvs} is usually employed to get ground truth poses \kp{nerf staff, 3D rendering; find an appropriate term, verify usage of COLMAP}. Likewise, COLMAP is also used as a ground truth acquisition method for VIO benchmarks \cite{} \kp{+1-2 more citations}. To our knowledge, there is no thorough study that compares pose estimation accuracy of existing SLAM and SfM methods \kp{is there?}, thus, to \kp{what for? motivation should be based on the examples above} we in addition to ORB-SLAM2 poses provide ground truth poses obtained from COLMAP 3D reconstructions. A COLMAP reconstruction is defined up to a scale factor so in order to get the metric scale for ground truth poses we \kp{Here describe alignment method and recovery of the scaling factor}

\kp{How do we treat each of the ground truth tracks (orb, colmap)? What is their intention? Which one to prioritize and why? Elaborate} 

To assess the accuracy of the ground truth poses we similar to \cite{} record several testing sequences in the laboratory environment where the use of a more accurate ground truth acquisition method is possible. In particular, we utilize OptiTrack MoCap system to record \kp{how much seqs do we have?} testing sequences. \kp{Adapt stuff from 4.4.2 here}

\kp{conclusions and error estimates based on the previous paragraph}

\kp{END}

Additionally, we deliver reference ground truth trajectories that were obtained with ORB-SLAM 3~\cite{campos2021orb} (RGBD modification) method~---State of The Art RGBD method on a wide variety of benchmark datasets~\cite{zhang2021survey}. In our variant, it uses RGB information from the smartphone and depth information from the external depth camera, re-projected onto smartphone coordinate frame, using calibrated intrinsics and extrinsics from Sec.~\ak{add}. In this section, we explain the motivation for using ORB SLAM and provide quantitative results on the quality of trajectories.

\subsubsection{Motivation on ORB-SLAM}

The de-facto standard tool for calculating camera poses for further usage in dense 3D reconstruction or rendering tasks is extrinsic parameters from sparse reconstruction step of COLMAP~\cite{schoenberger2016sfm, schoenberger2016mvs}. It is based on Bundle Adjustment and SIFT features; both of these components introduce significant computational complexity and border close to real-time performance. Additionally, COLMAP doesn't provide proper scaling to real-world coordinates \ak{why, explain}. Considering those properties and the high accuracy of RGBD modification of ORB SLAM on a wide variety of data, we considered it the main contender for COLMAP.

\subsubsection{Full-reference evaluation}

To compare quality of trajectories from ORB SLAM 3 and COLMAP, we recorded 5 records of one person in common dataset format using OptiTrack motion capture system~(mocap) as ground truth that provides sub-millimeter accuracy. Mocap was synchronized with the platform in offline by Twist-n-Sync algorithm~\cite{faizullin2021twist}. Since the algorithm is based on angular velocities analysis, the mocap velocity was extracted by finite difference of measured angle. ~\ak{MARSEL, name, accuracy, way to sync}\mf{DONE}. To calculate error statistics, we used implementation of Absolute Pose Error (APE) and Relative Pose Error (RPE) metrics from evo tool~\cite{grupp2017evo}. Before calculating APE, trajectories were aligned by Umeyama alignment. COLMAP trajectories were additionally scaled during Umeyama alignment. Because landmarks on person body are potentially dynamic (person can breath, blink), we considered three modifications of ORB SLAM -- not using person mask, using mask for background, using mask for person. Tab.~\ref{fig:eval_mocap} presents results of evaluation those ORB SLAM variants and COLMAP.

\ak{Explain why we don't provide APE-rot}

\ak{Results: ORB outperforms COLMAP on RPE for both rotation and translation. COLMAP with scaling outperforms ORB on APE because scaling overfits error, ORB with scaling gives comparable results (here maps from pcs could be demonstrated). Masks doesn't help, but on background they are comparable to original one. }

\begin{table}
  \centering
  \begin{tabular}{@{}lccr@{}}
    \toprule
    Method & APE-transl & RPE-rot & RPE-transl \\
    \midrule
    & Record 1 & & \\
    \midrule
    ORB & 0.0155 &	3.8390 & 0.0252 \\
    ORB (person) & 0.0192 &	3.8629	 & 0.0286 \\
    ORB (background) & 0.0290 &	3.8450 & 0.0263 \\
    COLMAP (with scaling) & 0.0073 &	3.8466	 & 0.0251 \\
    ORB (with scaling) & 0.0071 &	3.8390 & 0.0249 \\
    ORB + ICP & 0.0102 &	3.8274 & 0.0248 \\
    \midrule
    & Record 2 & & \\
    \midrule
    ORB &	0.0108 &	3.9622 &	0.0247 \\
    ORB (person) &	0.0182 &	3.9753 &	0.0262 \\
    ORB (background) &	0.0199 &	3.9767 &	0.0255 \\
    COLMAP (with scaling) &	0.0077 &	3.9751 &	0.0246 \\
    ORB (with scaling) &	0.0075 &	3.9622 &	0.0245 \\
    ORB + ICP ref &	0.0065 &	3.9559 &	0.0244 \\
    \midrule
    & Record 3 & & \\
    \midrule
    ORB &	0.0089 &	4.2945 &	0.0250 \\
    ORB (person) &	0.0150 &	4.3125 &	0.0275 \\
    ORB (background) &	0.0226 &	4.3302 &	0.0271 \\
    COLMAP (with scaling) &	0.0091 &	4.2977 &	0.0252 \\
    ORB (with scaling) &	0.0086 &	4.2945 &	0.0249 \\
    ORB + ICP ref &	0.0106 &	4.2996 &	0.0248 \\
        \midrule
    & Record 4 & & \\
    \midrule
    ORB &	0.0115 &	5.0057 &	0.0405 \\
    ORB (person) & - &	- &	- \\
    ORB (background) &	0.0247 &	5.0268 &	0.0409 \\
    COLMAP (with scaling) &	0.0070 &	5.0183 &	0.0403 \\
    ORB (with scaling) &	0.0067 &	5.0057 &	0.0400 \\
    ORB + ICP ref &	0.0055 &	5.0028 &	0.0402 \\
        \midrule
    & Record 5 & & \\
    \midrule
    ORB &	0.0095 &	4.9295 &	0.0368 \\
    ORB (person) &	0.3196 &	5.4726 &	0.0823 \\
    ORB (background) &	0.0180 &	4.9435 &	0.0371 \\
    COLMAP (with scaling) &	0.0053 &	4.9371 &	0.0367 \\
    ORB (with scaling) &	0.0053 &	4.9295 &	0.0364 \\
    ORB + ICP ref &	0.0056 &	4.9336 &	0.0368 \\
    \bottomrule
  \end{tabular}
  \caption{Eval}
  \label{tab:eval_mocap}
\end{table}

\subsubsection{Scaling trajectories}



==> src/trash.tex <==

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lccr@{}}
%     \toprule
%     Method & APE-transl & RPE-rot & RPE-transl \\
%     \midrule
%     & Record 1 & & \\
%     \midrule
%     ORB & 0.0155 &	3.8390 & 0.0252 \\
%     ORB (person) & 0.0192 &	3.8629	 & 0.0286 \\
%     ORB (background) & 0.0290 &	3.8450 & 0.0263 \\
%     COLMAP (with scaling) & 0.0073 &	3.8466	 & 0.0251 \\
%     ORB (with scaling) & 0.0071 &	3.8390 & 0.0249 \\
%     ORB + ICP & 0.0102 &	3.8274 & 0.0248 \\
%     \midrule
%     & Record 2 & & \\
%     \midrule
%     ORB &	0.0108 &	3.9622 &	0.0247 \\
%     ORB (person) &	0.0182 &	3.9753 &	0.0262 \\
%     ORB (background) &	0.0199 &	3.9767 &	0.0255 \\
%     COLMAP (with scaling) &	0.0077 &	3.9751 &	0.0246 \\
%     ORB (with scaling) &	0.0075 &	3.9622 &	0.0245 \\
%     ORB + ICP ref &	0.0065 &	3.9559 &	0.0244 \\
%     \midrule
%     & Record 3 & & \\
%     \midrule
%     ORB &	0.0089 &	4.2945 &	0.0250 \\
%     ORB (person) &	0.0150 &	4.3125 &	0.0275 \\
%     ORB (background) &	0.0226 &	4.3302 &	0.0271 \\
%     COLMAP (with scaling) &	0.0091 &	4.2977 &	0.0252 \\
%     ORB (with scaling) &	0.0086 &	4.2945 &	0.0249 \\
%     ORB + ICP ref &	0.0106 &	4.2996 &	0.0248 \\
%         \midrule
%     & Record 4 & & \\
%     \midrule
%     ORB &	0.0115 &	5.0057 &	0.0405 \\
%     ORB (person) & - &	- &	- \\
%     ORB (background) &	0.0247 &	5.0268 &	0.0409 \\
%     COLMAP (with scaling) &	0.0070 &	5.0183 &	0.0403 \\
%     ORB (with scaling) &	0.0067 &	5.0057 &	0.0400 \\
%     ORB + ICP ref &	0.0055 &	5.0028 &	0.0402 \\
%         \midrule
%     & Record 5 & & \\
%     \midrule
%     ORB &	0.0095 &	4.9295 &	0.0368 \\
%     ORB (person) &	0.3196 &	5.4726 &	0.0823 \\
%     ORB (background) &	0.0180 &	4.9435 &	0.0371 \\
%     COLMAP (with scaling) &	0.0053 &	4.9371 &	0.0367 \\
%     ORB (with scaling) &	0.0053 &	4.9295 &	0.0364 \\
%     ORB + ICP ref &	0.0056 &	4.9336 &	0.0368 \\
%     \bottomrule
%   \end{tabular}
%   \caption{Eval}
%   \label{tab:eval_mocap}
% \end{table}


% \subsubsection{Motivation on ORB-SLAM}

% The de-facto standard tool for calculating camera poses for further usage in dense 3D reconstruction or rendering tasks is extrinsic parameters from sparse reconstruction step of COLMAP~\cite{schoenberger2016sfm, schoenberger2016mvs}. It is based on Bundle Adjustment and SIFT features; both of these components introduce significant computational complexity and border close to real-time performance. Additionally, COLMAP doesn't provide proper scaling to real-world coordinates \ak{why, explain}. Considering those properties and the high accuracy of RGBD modification of ORB SLAM on a wide variety of data, we considered it the main contender for COLMAP.

% \subsubsection{Full-reference evaluation}

% To compare quality of trajectories from ORB SLAM 3 and COLMAP, we recorded 5 records of one person in common dataset format using OptiTrack motion capture system~(mocap) as ground truth that provides sub-millimeter accuracy. Mocap was synchronized with the platform in offline by Twist-n-Sync algorithm~\cite{faizullin2021twist}. Since the algorithm is based on angular velocities analysis, the mocap velocity was extracted by finite difference of measured angle. ~\ak{MARSEL, name, accuracy, way to sync}\mf{DONE}. To calculate error statistics, we used implementation of Absolute Pose Error (APE) and Relative Pose Error (RPE) metrics from evo tool~\cite{grupp2017evo}. Before calculating APE, trajectories were aligned by Umeyama alignment. COLMAP trajectories were additionally scaled during Umeyama alignment. Because landmarks on person body are potentially dynamic (person can breath, blink), we considered three modifications of ORB SLAM -- not using person mask, using mask for background, using mask for person. Tab.~\ref{fig:eval_mocap} presents results of evaluation those ORB SLAM variants and COLMAP.

% \ak{Explain why we don't provide APE-rot}

% \ak{Results: ORB outperforms COLMAP on RPE for both rotation and translation. COLMAP with scaling outperforms ORB on APE because scaling overfits error, ORB with scaling gives comparable results (here maps from pcs could be demonstrated). Masks doesn't help, but on background they are comparable to original one. }

% \subsubsection{Scaling trajectories}

\ak{Motivation on SfM and RGBD}
\textbf{RGBD}  \kp{why it is important? because nerfs and other our applications (which?) like good poses; need to elaborate with references}. In our implementation, we use RGB modification of ORB-SLAM3 \cite{campos2021orb} that works in the same way as ORB-SLAM2 \kp{right?}. We provide RGB frames and depth information to the algorithm from the smartphone and from the external depth camera respectively. Depth frames are transformed to the RGB frames reference system of coordinates using the calibration (see section \ref{sec:calib_cam2depth}).
\kp{A few words about BundleFusion?}

\textbf{SfM} In the area of 3D reconstruction that the proposed dataset is aimed at, a Structure-from-Motion (SfM) pipeline COLMAP \cite{schoenberger2016sfm, schoenberger2016mvs} is usually employed to get ground truth poses \kp{nerf staff, 3D rendering; find an appropriate term, verify usage of COLMAP}. Likewise, COLMAP is also used as a ground truth acquisition method for VIO benchmarks \cite{} \kp{+1-2 more citations}. To our knowledge, there is no thorough study that compares pose estimation accuracy of existing SLAM and SfM. A COLMAP reconstruction  so in order to get the metric scale for ground truth poses we \kp{Here describe alignment method and recovery of the scaling factor}

% \kp{How do we treat each of the ground truth tracks (orb, colmap)? What is their intention? Which one to prioritize and why? Elaborate} 

%  \kp{Adapt stuff from 4.4.2 here}

% \kp{conclusions and error estimates based on the previous paragraph}

% Additionally, we deliver reference ground truth trajectories that were obtained with ORB-SLAM 3~\cite{campos2021orb} (RGBD modification) method~---State of The Art RGBD method on a wide variety of benchmark datasets~\cite{zhang2021survey}. In our variant, it uses RGB information from the smartphone and depth information from the external depth camera, re-projected onto smartphone coordinate frame, using calibrated intrinsics and extrinsics from Sec.~\ak{add}. In this section, we explain the motivation for using ORB SLAM and provide quantitative results on the quality of trajectories.


%\begin{table}
%  \fontsize{9.5}{9}\selectfont
%  \centering
%  \begin{tabular}{@{}lcr@{}}
%    \toprule
%    Type & Data & Properties \\
%    \midrule
%    Smartphone & RGB video & 1920 $\times$ 1080, 30 Hz \\
%    & Gyroscope & , 500 Hz \\
%    & Accelerometer & , 500 Hz \\
%    & Flash timestamps & \ak{??}, 1 Hz \\ 
%    % \midrule
%    Depth camera & Depth frames & 640 $\times$ 576, 5 Hz \\
%    \midrule
%    Segment. masks & RGB video & 1920 $\times$ 1080, 30 Hz \\
%    % \midrule
%    Ground truth & 3D poses & 5 Hz \\
%    \bottomrule
%  \end{tabular}
%  \caption{Recorded data \gf{what is new wrt the table at RW?}}
%  \label{tab:dataset}
%\end{table}
